String Diagrams for Closed Symmetric Monoidal Categories

We introduce a graphical language for closed symmetric monoidal categories based on an extension of string diagrams with special bracket wires representing internal homs. These bracket wires make the structure of the internal hom functor explicit, allowing standard morphism wires to interact with them through a well-defined set of graphical rules. We establish the soundness and completeness of the diagrammatic calculus, and illustrate its expressiveness through examples drawn from category theory, logic and programming language semantics.

==> ClosedDiags/BigCupSplit/8.tex <==
\tikzsetnextfilename{ClosedDiags/BigCupSplit/8}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b0//0.5,
    b1//0.5,
    B//0.5,
    A//0.5,
    b2//1,
    b3//0.5,
    D//0.5,
    C//0.5,
    b4//0.5,
    b5//0
}


\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{2.5,-3}[right]
\bShift{b2}{2.5,-3}

\bShift{b3}{-2.5,-3}[right]
\bShift{b4}{-2.5,-3}

\bShift{b3}{0,-1.5}[right]
\bShift{b4}{0,-1.5}


\bCup{b1}{b2}
\bCup{b3}{b4}

\coord{b0}{b0}{0,-2}
\coord{b5}{b5}{0,-2}

\bCap{b0}{b5}[1.5]

\bShift{b0}{0,-1.5}[right]
\bShift{b5}{0,-1.5}

\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/CapBubbleCross/5.tex <==
\tikzsetnextfilename{ClosedDiags/CapBubbleCross/5}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=0.7]
\drawStartNodes{
    b1/ /2,
    b2//0
}

\coord{b1}{b1}{0,-1.5}
\coord{b2}{b2}{0,-1.5}

\coord{A1}{b1}{0.5,0}
\coord{B1}{b2}{-0.5,0}

\ddCap{A1}{B1}

\bCap{b1}{b2}[1]
\ddShift{B1}{0,-1}
\ddShift{B1}{0,-1}
\ddShift{B1}{0,-1}
\udShift{A1}{-0.5,-1}
\udShift{A1}{0,-1}
\udShift{A1}{0,-1}

\bShift{b1}{0.5,-1}[right]
\bShift{b2}{0,-1}

\bCup{b1}{b2}[0.75]


\drawEndNodes{
    A1/$X$/,
    B1/$X$/
}
\end{tikzpicture}


==> ClosedDiags/CellGen/fNormal.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/fNormal}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A/$X$/0
}

\ddShift{A}{0,-1}
\coord{B}{A}{0,0}
\ddShift{A}{0,-1}
\bead{B}{B}{f}
\coord{B}{B}{0,0.5}
\bead{B}{B}{\nu^{-1}}
\coord{B}{B}{0,-1}
\bead{B}{B}{\nu}

\drawEndNodes{
    A/$Y$
}
\end{tikzpicture}


==> ClosedDiags/CellGen/fUpNormal.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/fUpNormal}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A/$Y$/0
}

\udShift{A}{0,-1}
\coord{B}{A}{0,0}
\udShift{A}{0,-1}
\bead{B}{B}{f}
\coord{B}{B}{0,0.5}
\bead{B}{B}{\XYflip{\nu}}
\coord{B}{B}{0,-1}
\bead{B}{B}{\XYflip{\nu^{-1}}}
\drawEndNodes{
    A/$X$
}
\end{tikzpicture}


==> ClosedDiags/CellGen/tFlip.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/tFlip}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A/$Y$/0
}

\udShift{A}{0,-1}
\coord{B}{A}{0,0}
\udShift{A}{0,-1}
\bead{B}{B}{\Yflip{\flip{t}}}
\drawEndNodes{
    A/$X$
}
\end{tikzpicture}


==> ClosedDiags/CellGen/tUpBrackets.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/tUpBrackets}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    X//0.5,
    A//0.5,
    Y//0.5,
    b2//0
}
\sShift{X}{0,-1}
\sShift{X}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b2}{0,-1}
\bShift{b2}{0,-1}

\udShift{A}{0,-1}
\coord{B}{A}{0,0}
\udShift{A}{0,-1}
\bead{B}{B}{t}
\drawEndNodes{
    A/
}
\end{tikzpicture}


==> ClosedDiags/CellGen/tUpFlip.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/tUpFlip}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A/$X$/0
}
\ddShift{A}{0,-1}
\coord{B}{A}{0,0}
\ddShift{A}{0,-1}
\bead{B}{B}{\flip{\Yflip{t}}}
\drawEndNodes{
    A/$Y$
}
\end{tikzpicture}


==> ClosedDiags/CellGen/upDownCross.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/upDownCross}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A/$A$/0.5,
    B/$B$/0.5,
    C/$C$/0.5,
    D/$D$/0.5,
    b2//0
}

\bShift{b1}{0,-1}[right]
\sShift{A}{0,-1}
\udShift{B}{0.5,-1}
\ddShift{C}{-0.5,-1}
\sShift{D}{0,-1}
\bShift{b2}{0,-1}
\drawEndNodes{
    A/$A$,
    B/$B$,
    C/$C$,
    D/$D$
}
\end{tikzpicture}


==> ClosedDiags/CellGen/upUpCross.tex <==
\tikzsetnextfilename{ClosedDiags/CellGen/upUpCross}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A/$A$/0.5,
    B/$B$/0.5,
    C/$C$/0.5,
    D/$D$/0.5,
    b2//0
}

\bShift{b1}{0,-1}[right]
\sShift{A}{0,-1}
\udShift{B}{0.5,-1}
\udShift{C}{-0.5,-1}
\sShift{D}{0,-1}
\bShift{b2}{0,-1}
\drawEndNodes{
    A/$A$,
    B/$B$,
    C/$C$,
    D/$D$
}
\end{tikzpicture}


==> ClosedDiags/Currying/1.tex <==
\tikzsetnextfilename{ClosedDiags/Currying/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$A$}/0
}
\drawArrowShift{A}{0,-1}
\coordinate (B) at (A);
\drawArrowShift{B}{0,-1}
\bead{A}{A}{f}

\drawEndNodes{
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/Currying/2.tex <==
\tikzsetnextfilename{ClosedDiags/Currying/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]

\coordinate (A) at (0,0);
\coordinate (A1) at (-0.5,0);
\coordinate (b) at (-1,0);
\coordinate (b1) at (0.5,0);
\drawCap{A1}{A}[0.25]

\bracketCap{b}{b1}
\drawBracketShift{b}{0,-1}[right]
\drawBracketShift{b}{0,-1}[right]

\drawBracketShift{b1}{0,-1}
\drawBracketShift{b1}{0,-1}

\drawArrowShift{A}{0,-1}
\upArrowShift{A1}{0,-1}
\upArrowShift{A1}{0,-1}
\coordinate (B) at (A);
\drawArrowShift{B}{0,-1}

\bead{A}{A}{f}

\end{tikzpicture}


==> ClosedDiags/DecompProofs/cap/2.tex <==
\tikzsetnextfilename{ClosedDiags/DecompProofs/cap/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$X$}/3.5,
    B/{$Z$}/0.5,
    b4//0
}

\udShift{A}{0,-1}
\ddShift{B}{0,-1}

\coordinate[shift={(-0.5,0)}] (b3) at (B);
\coordinate[shift={(-1,0)}] (C2) at (B);
\coordinate[shift={(-1.5,0)}] (C1) at (B);
\coordinate[shift={(-2,0)}] (b2) at (B);

\ddCap{C1}{C2}[0.25]
\bCap{b2}{b3}[0.75]

\coordinate[shift={(-1,0)}] (C0) at (C1);
\coordinate[shift={(-1.5,0)}] (C00) at (C1);

\ddCup{C0}{C1}
\ddCap{C00}{C0}[0.25]

\bShift{b2}{0,-0.75}[right]
\bShift{b3}{0,-0.75}

\ddShift{B}{0,-1}
\ddShift{B}{0,-1}

\ddShift{C2}{0,-1}
\ddShift{C2}{0,-1}

\udShift{A}{0,-1}
\udShift{A}{0,-1}

\bCup{b2}{b3}[0.75]

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{C00}{0,-1}
\udShift{C00}{0,-1}

\drawEndNodes{
    A/{$X$},
    C2/{$Y$},
    C00/{$Y$},
    B/{$Z$}
}
\end{tikzpicture}


==> ClosedDiags/DecompProofs/cap/3.tex <==
\tikzsetnextfilename{ClosedDiags/DecompProofs/cap/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$X$}/2.5,
    B/{$Z$}/0.5,
    b4//0
}

\udShift{A}{0,-1}
\ddShift{B}{0,-1}

\coordinate[shift={(-0.5,0)}] (b3) at (B);
\coordinate[shift={(-1,0)}] (b2) at (B);

\bCap{b2}{b3}[0.25]

\coordinate[shift={(-1.5,0)}] (C0) at (B);
\coordinate[shift={(-2,0)}] (C00) at (B);

\ddCap{C00}{C0}[0.25]

\ddShift{C0}{0.5,-1}

\bShift{b2}{-0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{B}{0,-1}
\ddShift{B}{0,-1}


\udShift{A}{0,-1}
\udShift{A}{0,-1}

\ddShift{C0}{0,-1}

\bCup{b2}{b3}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{C00}{0,-1}
\udShift{C00}{0,-1}

\drawEndNodes{
    A/{$X$},
    C0/{$Y$},
    C00/{$Y$},
    B/{$Z$}
}
\end{tikzpicture}


==> ClosedDiags/Generators/10.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/10}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    s1//0.5,
    A//1,
    B//0.5,
    s2//0.5,
    b2//0
}
\coordinate[shift={(0,-1)}] (A) at (A);
\coordinate[shift={(0,-1)}] (B) at (B);

\sShift{s1}{0,-1}
\sShift{s2}{0,-1}

\bShift{b1}{0,-1}[right]
\ddbCap{B}{A}
\bShift{b2}{0,-1}

\drawEndNodes{
    s2//
}
\end{tikzpicture}


==> ClosedDiags/Generators/11.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/11}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}

\ddShift{A}{0,-1}
\bCup{b1}{b2}

\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/Generators/12.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/12}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}
\coordinate[shift={(0,-1)}] (b1) at (b1);
\coordinate[shift={(0,-1)}] (b2) at (b2);

\ddShift{A}{0,-1}
\bCap{b1}{b2}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/Generators/14.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/14}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}

\bbCup{b2}{b3}
\ddbCup{C}{B}[1]

\sShift{A}{0,-1}
\sShift{D}{0,-1}
\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/Generators/2.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    B//0.5,
    b2//0.5,
    A//0
}

\bShift{b1}{0,-1}[right]
\sShift{B}{0,-1}
\ddShift{A}{-0.5,-1}
\bShift{b2}{0.5,-1}

\drawEndNodes{
    A//,
    B//
}

\end{tikzpicture}


==> ClosedDiags/Generators/2a.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/2a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    B//0.5,
    A//0.5,
    b2//0
}

\bShift{b1}{0,-1}[right]
\ddShift{B}{0,-1}
\ddShift{A}{0.5,-1}
\bShift{b2}{-0.5,-1}

\drawEndNodes{
    A//,
    B//
}

\end{tikzpicture}


==> ClosedDiags/Generators/4.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/4}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    B//0.5,
    A//0.5,
    b2//0.5,
    C//0
}

\bShift{b1}{0,-1}[right]
\sShift{B}{0,-1}
\ddbCup{C}{A}
\bShift{b2}{0,-1}

\drawEndNodes{
    B//
}

\end{tikzpicture}


==> ClosedDiags/Generators/6.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/6}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    s1//0.5,
    b2//0.5,
    s2//0.5,
    A//0.5,
    b3//0.5,
    s3//0.5,
    b4//0
}
\sShift{s1}{0,-1}
\sShift{s2}{0,-1}
\sShift{s3}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\udShift{A}{0.5,-1}
\bShift{b3}{-0.5,-1}
\bShift{b4}{0,-1}


\drawEndNodes{
    s2//
}
\end{tikzpicture}


==> ClosedDiags/Generators/8.tex <==
\tikzsetnextfilename{ClosedDiags/Generators/8}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    s1//0.5,
    b2//0.5,
    s2//0.5,
    b3//0.5,
    A//0.5,
    s3//0.5,
    b4//0
}
\ddShift{s1}{0,-1}
\sShift{s2}{0,-1}
\ddShift{s3}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\udShift{A}{-0.5,-1}
\bShift{b3}{0.5,-1}
\bShift{b4}{0,-1}


\drawEndNodes{
    s2/c/
}
\end{tikzpicture}


==> ClosedDiags/GeneratorsBaseline/11a.tex <==
\tikzsetnextfilename{ClosedDiags/GeneratorsBaseline/11a}
\begin{tikzpicture}[baseline={(current bounding box.north)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}

\bCup{b1}{b2}
\coord{b1}{b1}{0,-1}

\drawEndNodes{b1/}

\end{tikzpicture}


==> ClosedDiags/GeneratorsBaseline/12a.tex <==
\tikzsetnextfilename{ClosedDiags/GeneratorsBaseline/12a}
\begin{tikzpicture}[baseline={(current bounding box.north)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}
\coordinate[shift={(0,-1)}] (b1) at (b1);
\coordinate[shift={(0,-1)}] (b2) at (b2);
\bCap{b1}{b2}

\drawEndNodes{b1/}

\end{tikzpicture}


==> ClosedDiags/Local/1.tex <==
\tikzsetnextfilename{ClosedDiags/Local/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0.5,
C//0.5,
D//0.5,
b1//1,
b2//0.5,
E//0.5,
F//0.5,
G//0.5,
b3//0.5,
H//0.5
}

\bShift{b0}{0,-1}[right]
\bShift{b1}{0,-1}
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b3}{0,-1}


\bbCup{b1}{b2}

\sShift{A}{0,-0.5}
\sShift{B}{0,-0.5}
\sShift{G}{0,-0.5}
\sShift{H}{0,-0.5}

\sShift{C}{0,-1}
\sShift{C}{0,-1}
\ddShift{D}{0,-1}
\udShift{E}{0,-1}
\sShift{F}{0,-1}
\sShift{F}{0,-1}

\ddCup{D}{E}[1]

\coord{A1}{A}{0,0}
\coord{B1}{B}{0,0}
\coord{G1}{G}{0,0}
\coord{H1}{H}{0,0}

\bShift{b0}{0,-1}[right]
\sShift{A}{0,-1.5}
\sShift{B}{0,-1.5}
\sShift{G}{0,-1.5}
\sShift{H}{0,-1.5}

\dashbead{A1}{B1}
\dashbead{G1}{H1}

\end{tikzpicture}


==> ClosedDiags/Local/10.tex <==
\tikzsetnextfilename{ClosedDiags/Local/10}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    B//0.5,
    b//0.5,
    A//0
}

\ddCup{B}{A}
\bShift{b}{0,-1}[right]

\drawEndNodes{b/}

\end{tikzpicture}


==> ClosedDiags/Local/1a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/1a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0.5,
C//0.5,
D//0.5,
b1//1,
b2//0.5,
E//0.5,
F//0.5,
b3//0
}

\coord{C1}{C}{0,-0.75}
\coord{F1}{F}{0,-0.75}

\bShift{b1}{0,-1}
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b3}{0,-1}


\bbCup{b1}{b2}

\ddCup{A}{B}
\bShift{b0}{0,-1}[right]

\sShift{C}{0,-1}
\sShift{C}{0,-1}
\ddShift{D}{0,-1}
\udShift{E}{0,-1}
\sShift{F}{0,-1}
\sShift{F}{0,-1}

\ddCup{D}{E}[1]


\bShift{b0}{0,-1}[right]

\bead{C1}{C1}{t}
\bead{F1}{F1}{t}


\end{tikzpicture}


==> ClosedDiags/Local/2.tex <==
\tikzsetnextfilename{ClosedDiags/Local/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0.5,
C//0.5,
D//0.5,
b1//1,
b2//0.5,
E//0.5,
F//0.5,
G//0.5,
b3//0.5,
H//0
}

\bShift{b0}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b3}{0,-1}

\bbCup{b1}{b2}

\sShift{A}{0,-1.5}
\sShift{B}{0,-1.5}

\sShift{G}{0,-1.5}
\sShift{H}{0,-1.5}

\sShift{C}{0,-1}
\sShift{C}{0,-1}
\sShift{F}{0,-1}
\sShift{F}{0,-1}

\ddCup{D}{E}[1]

\coord{A1}{A}{0,0}
\coord{B1}{B}{0,0}

\coord{G1}{G}{0,0}
\coord{H1}{H}{0,0}

\bShift{b0}{0,-1}[right]
\sShift{A}{0,-0.5}
\sShift{B}{0,-0.5}

\sShift{G}{0,-0.5}
\sShift{H}{0,-0.5}


\dashbead{A1}{B1}

\dashbead{G1}{H1}


\end{tikzpicture}


==> ClosedDiags/Local/2a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/2a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0.5,
C//0.5,
D//0.5,
b1//1,
b2//0.5,
E//0.5,
F//0.5,
b3//0
}

\bShift{b0}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b3}{0,-1}


\bbCup{b1}{b2}

\ddShift{A}{0,-1}
\udShift{B}{0,-1}
\sShift{C}{0,-1}
\sShift{C}{0,-1}
\sShift{F}{0,-1}
\sShift{F}{0,-1}

\ddCup{A}{B}[0.4]
\ddCup{D}{E}[1]

\coord{A1}{A}{0,0}
\coord{B1}{B}{0,0}

\bShift{b0}{0,-1}[right]

\coord{C1}{C}{0,0.4}
\coord{F1}{F}{0,0.4}

\bead{C1}{C1}{t}
\bead{F1}{F1}{t}


\end{tikzpicture}


==> ClosedDiags/Local/3.tex <==
\tikzsetnextfilename{ClosedDiags/Local/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0
}

\bShift{b0}{0,-1}[right]

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coord{A1}{A}{0,0}
\coord{B1}{B}{0,0}


\bShift{b0}{0,-1}[right]

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\dashbead{A1}{B1}

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/3a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/3a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0
}

\bShift{b0}{0,-1}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coord{A1}{A}{0,0}
\coord{B1}{B}{0,0}


\bShift{b0}{0,-1}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\dashbead{A1}{B1}

\drawEndNodes{A/}
]

\end{tikzpicture}


==> ClosedDiags/Local/6.tex <==
\tikzsetnextfilename{ClosedDiags/Local/6}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b//0.5,
    A//0
}

\ddShift{A}{-0.5,-1}
\bShift{b}{0.5,-1}[right]

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/6a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/6a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A//0.5,
    b//0
}

\ddShift{A}{0.5,-1}
\bShift{b}{-0.5,-1}

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/7.tex <==
\tikzsetnextfilename{ClosedDiags/Local/7}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b//0.5,
    A//0
}

\udShift{A}{-0.5,-1}
\bShift{b}{0.5,-1}[right]

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/7a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/7a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A//0.5,
    b//0
}

\udShift{A}{0.5,-1}
\bShift{b}{-0.5,-1}

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/8.tex <==
\tikzsetnextfilename{ClosedDiags/Local/8}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A//0.5,
    b//0
}

\udShift{A}{0.5,-1}
\bShift{b}{-0.5,-1}[right]

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/8a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/8a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b//0.5,
    A//0
}

\udShift{A}{-0.5,-1}
\bShift{b}{0.5,-1}

\drawEndNodes{A/}

\end{tikzpicture}


==> ClosedDiags/Local/9.tex <==
\tikzsetnextfilename{ClosedDiags/Local/9}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b//0
}

\bShift{b}{0,-1}[right]

\drawEndNodes{b/}

\end{tikzpicture}


==> ClosedDiags/Local/9a.tex <==
\tikzsetnextfilename{ClosedDiags/Local/9a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b//0
}

\bShift{b}{0,-1}

\drawEndNodes{b/}

\end{tikzpicture}


==> ClosedDiags/NormalProof/notation1.tex <==
\tikzsetnextfilename{ClosedDiags/NormalProof/notation1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    X/$\hat{X}$/0
}

\ddShift{X}{0,-1}

\drawEndNodes{
    X/$\hat{X}$
}
\end{tikzpicture}


==> ClosedDiags/NormalProof/notation2.tex <==
\tikzsetnextfilename{ClosedDiags/NormalProof/notation2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    X/$\check{X}$/0
}

\udShift{X}{0,-1}

\drawEndNodes{
    X/$\check{X}$
}
\end{tikzpicture}


==> ClosedDiags/Normaliser/1b.tex <==
\tikzsetnextfilename{ClosedDiags/Normaliser/1b}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    X/$X$/0
}

\ddShift{X}{0,-1}
\coord{X1}{X}{0,0}

\ddShift{X}{0,-1}

\bead{X1}{X1}{\nu}

\drawEndNodes{
    X/${\bar{X}}$
}
\end{tikzpicture}


==> ClosedDiags/Normaliser/1c.tex <==
\tikzsetnextfilename{ClosedDiags/Normaliser/1c}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    X/$X$/0
}

\udShift{X}{0,-1}
\coord{X1}{X}{0,0}

\udShift{X}{0,-1}

\bead{X1}{X1}{\nu}

\drawEndNodes{
    X/$\bar{X}$
}
\end{tikzpicture}


==> ClosedDiags/Normaliser/2a.tex <==
\tikzsetnextfilename{ClosedDiags/Normaliser/2a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    X//1.5,
    Y//0.5,
    b2//0
}

\sShift{X}{0,-1}
\sShift{X}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}


\end{tikzpicture}


==> ClosedDiags/Normaliser/2b.tex <==
\tikzsetnextfilename{ClosedDiags/Normaliser/2b}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    X1//0.5,
    X2//0
}


\coord{X1}{X1}{0,-1}
\coord{X2}{X2}{0,-1}

\coord{X11}{X1}{0,0}
\coord{X21}{X2}{0,0}

\udShift{X1}{0,-1}
\ddShift{X2}{0,-1}

\bead{X11}{X21}{\nu}

\drawEndNodes{
    X1
}


\end{tikzpicture}


==> ClosedDiags/Normaliser/2c.tex <==
\tikzsetnextfilename{ClosedDiags/Normaliser/2c}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    X//1.5,
    Y//0.5,
    b2//0
}

\sShift{X}{0,-1}
\sShift{X}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}

\end{tikzpicture}


==> ClosedDiags/Primitives/1.tex <==
\tikzsetnextfilename{ClosedDiags/Primitives/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    g/{}/1,
    f/{$A$}/0
}

\drawArrowShift{f}{-1,-1}
\drawBracketShift{g}{1,-1}

\drawEndNodes{
    f/$A$
}
\end{tikzpicture}


==> ClosedDiags/Primitives/2.tex <==
\tikzsetnextfilename{ClosedDiags/Primitives/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    g/{}/1,
    f/{$A$}/0
}

\upArrowShift{f}{-1,-1}
\leftBracketShift{g}{1,-1}

\drawEndNodes{
    f/$A$
}
\end{tikzpicture}


==> ClosedDiags/Primitives/3.tex <==
\tikzsetnextfilename{ClosedDiags/Primitives/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    f/{$A$}/1,
    g/{$A$}/0
}
\drawCup{f}{g}

\end{tikzpicture}


==> ClosedDiags/Primitives/4.tex <==
\tikzsetnextfilename{ClosedDiags/Primitives/4}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    f/{}/1,
    g/{}/0
}
\coordinate[shift={(0,-1)}] (f) at (f);
\coordinate[shift={(0,-1)}] (g) at (g);
\drawCap{f}{g}

\drawEndNodes{
    f/$A$,
    g/$A$
}
\end{tikzpicture}


==> ClosedDiags/Primitives/5.tex <==
\tikzsetnextfilename{ClosedDiags/Primitives/5}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1/{}/0.5,
    f/{$A$}/0.5,
    b2/{}/0
}
\drawArrowShift{f}{0,-1}
\bracketCup{b1}{b2}

\drawEndNodes{
    f/{$A$}
}

\end{tikzpicture}


==> ClosedDiags/Primitives/6.tex <==
\tikzsetnextfilename{ClosedDiags/Primitives/6}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1/{}/0.5,
    A/{$A$}/0.5,
    b2/{}/0
}
\drawArrowShift{A}{(0,-1)}
\coordinate[shift={(0,-1)}] (b1) at (b1);
\coordinate[shift={(0,-1)}] (b2) at (b2);
\bracketCap{b1}{b2}

\drawEndNodes{
    A/{$A$}
}
\end{tikzpicture}


==> ClosedDiags/Rel/bubbleYank3.tex <==
\tikzsetnextfilename{ClosedDiags/Rel/bubbleYank3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=0.7
]
\drawStartNodes{
b1//1,
b2//1,
b3//0
}
\bShift{b1}{0,-1}
\coord{b2}{b2}{0,-1}
\coord{b3}{b3}{0,-1}

\bCap{b2}{b3}

\bbCup{b1}{b2}


\bShift{b3}{0,-1}


\drawEndNodes{
    b3//
}


\end{tikzpicture}


==> ClosedDiags/Rel/bubbleYank4.tex <==
\tikzsetnextfilename{ClosedDiags/Rel/bubbleYank4}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=0.8
]
\drawStartNodes{
b1//0
}

\bShift{b1}{0,-1}
\bShift{b1}{0,-1}


\drawEndNodes{
    b1//
}


\end{tikzpicture}


==> ClosedDiags/Rel/smooth2A.tex <==
\tikzsetnextfilename{ClosedDiags/Rel/smooth2A}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
b1//0.5,
A//1,
B//0.5,
b4//0
}

\ddShift{A}{0,-1}
\ddShift{B}{0,-1}
\ddShift{A}{0,-1}
\ddShift{B}{0,-1}

\coord{b1}{b1}{0,-2}
\coord{b4}{b4}{0,-2}
\bCap{b1}{b4}[1]


\end{tikzpicture}


==> ClosedDiags/Relations/Natural/3.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/Natural/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A//0.5,
    b1//0.5,
    B//0.5,
    C//0.5,
    b2//0
}

\ddShift{A}{0,-1}
\bShift{b1}{0,-1}[right]
\udShift{B}{0,-1}
\bShift{b2}{0,-1}
\sShift{C}{0,-1}

\coord{A1}{A}{0,0.5}
\coord{B1}{C}{0,0.5}

\ddCup{A}{B}{0.5,-1}
\bShift{b1}{0,-1}[right]
\sShift{C}{0,-1}
\bShift{b2}{0,-1}

\bead{A1}{A1}{t}
\bead{B1}{B1}{t}

\drawEndNodes{
    C//
}
\end{tikzpicture}


==> ClosedDiags/Relations/Natural/3a.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/Natural/3a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A//0.5,
    b1//0.5,
    B//0.5,
    C//0.5,
    b2//0
}

\ddShift{A}{0,-1}
\bShift{b1}{0,-1}[right]
\udShift{B}{0,-1}
\bShift{b2}{0,-1}
\sShift{C}{0,-1}

\coord{A1}{B}{0,0.5}

\ddCup{A}{B}{0.5,-1}
\bShift{b1}{0,-1}[right]
\sShift{C}{0,-1}
\bShift{b2}{0,-1}

\coord{B1}{C}{0,0.5}

\bead{A1}{A1}{t}
\bead{B1}{B1}{t}

\drawEndNodes{
    C//
}
\end{tikzpicture}


==> ClosedDiags/Relations/Natural/6.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/Natural/6}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    s1//0.5,
    A//1,
    B//0.5,
    s2//0.5,
    b2//0
}
\coordinate[shift={(0,-2)}] (A) at (A);
\coordinate[shift={(0,-2)}] (B) at (B);

\coord{S1}{s1}{0,-0.5}
\coord{S2}{s2}{0,-0.5}

\sShift{s1}{0,-1}
\sShift{s2}{0,-1}
\sShift{s1}{0,-1}
\sShift{s2}{0,-1}
\sShift{s1}{0,-1}
\sShift{s2}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\ddCap{A}{B}
\udShift{A}{0,-1}
\ddShift{B}{0,-1}

\coord{A1}{A}{0,0.5}

\bShift{b2}{0,-1}
\bShift{b2}{0,-1}
\bShift{b2}{0,-1}

\bead{A1}{A1}{t}
\bead{S1}{S1}{t}
\bead{S2}{S2}{t}


\drawEndNodes{
    s2//
}
\end{tikzpicture}


==> ClosedDiags/Relations/Natural/6a.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/Natural/6a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    s1//0.5,
    A//1,
    B//0.5,
    s2//0.5,
    b2//0
}
\coordinate[shift={(0,-2)}] (A) at (A);
\coordinate[shift={(0,-2)}] (B) at (B);

\coord{S1}{s1}{0,-2.5}
\coord{S2}{s2}{0,-2.5}

\sShift{s1}{0,-1}
\sShift{s2}{0,-1}
\sShift{s1}{0,-1}
\sShift{s2}{0,-1}
\sShift{s1}{0,-1}
\sShift{s2}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\ddCap{A}{B}
\udShift{A}{0,-1}
\ddShift{B}{0,-1}

\coord{B1}{B}{0,0.5}

\bShift{b2}{0,-1}
\bShift{b2}{0,-1}
\bShift{b2}{0,-1}

\bead{B1}{B1}{t}
\bead{S1}{S1}{t}
\bead{S2}{S2}{t}


\drawEndNodes{
    s2//
}
\end{tikzpicture}


==> ClosedDiags/Relations/SymEntry1.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/SymEntry1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$A$}/0.5,
    b1//0.5,
    s//0.5,
    b2//0
}
\udShift{A}{0.5,-1}
\drawBracketShift{b1}{-0.5,-1}[right]
\drawBracketShift{b1}{0,-1}[right]
\drawBracketShift{b1}{0,-1}[right]

\sShift{s}{0,-1}
\udShift{A}{0.5,-1}
\sShift{s}{-0.5,-1}
\sShift{s}{0,-1}

\drawBracketShift{b2}{0,-1}
\drawBracketShift{b2}{0,-1}
\udShift{A}{0.5,-1}
\drawBracketShift{b2}{-0.5,-1}

\drawEndNodes{
    A/{$A$}
}

\end{tikzpicture}


==> ClosedDiags/Relations/SymEntry2.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/SymEntry2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$A$}/0.5,
    b1//0.5,
    s//0.5,
    b2//0
}
\drawBracketShift{b1}{-0.5,-3}[right]
\drawBracketShift{b2}{-0.5,-3}
\sShift{s}{-0.5,-3}

\udShift{A}{1.5,-3}

\drawEndNodes{
    A/{$A$}
}

\end{tikzpicture}


==> ClosedDiags/Relations/cupNat4a.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/cupNat4a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
A//0.5,
b0//0.5,
B//0
}

\bShift{b0}{0,-1}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coord{A1}{A}{0,0}
\coord{B1}{B}{0,0}


\bShift{b0}{0,-1}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\dashbead{A1}{B1}

\end{tikzpicture}


==> ClosedDiags/Relations/pop1.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/pop1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1/{}/0.5,
    A/{$A$}/0.5,
    b2/{}/0
}
\coordinate[shift={(0,-1)}] (b1) at (b1);
\coordinate[shift={(0,-1)}] (b2) at (b2);
\bracketCap{b1}{b2}
\bracketCup{b1}{b2}

\drawArrowShift{A}{0,-1}
\drawArrowShift{A}{0,-1}

\drawEndNodes{
    A/$A$
}
\end{tikzpicture}


==> ClosedDiags/Relations/pop2.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/pop2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1,framed, background rectangle/.style={draw=black, dashed}]
\drawStartNodes{
    b1/{}/0.5,
    A/{}/0.5,
    b2/{}/0
}
\bracketCap{b1}{b2}[0.5][white]
\bracketCup{b1}{b2}[0.5][white]
\end{tikzpicture}


==> ClosedDiags/Relations/pop2a.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/pop2a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A/{$A$}/0
}


\drawArrowShift{A}{0,-1}
\drawArrowShift{A}{0,-1}

\drawEndNodes{
    A/$A$
}
\end{tikzpicture}


==> ClosedDiags/Relations/so1.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/so1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b/{}/0.5,
    B/{$B$}/0.5,
    b2/{}/0.5,
    f/{$A$}/0
}

\drawArrowShift{f}{-0.5,-1}
\drawArrowShift{B}{0,-1}
\drawBracketShift{b}{0,-1}[right]
\drawBracketShift{b2}{0.5,-1}
\drawArrowShift{f}{0,-1}
\drawArrowShift{B}{0,-1}
\bracketCup{b}{b2}

\drawEndNodes{
    f/$A$,
    B/$B$
}
\end{tikzpicture}


==> ClosedDiags/Relations/so2.tex <==
\tikzsetnextfilename{ClosedDiags/Relations/so2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b/{}/0.5,
    B/{$B$}/0.5,
    b2/{}/0.5,
    f/{$A$}/0
}

\drawArrowShift{f}{0,-1}
\drawArrowShift{B}{0,-1}
\drawBracketShift{b}{0,-1}[right]
\drawBracketShift{b2}{0,-1}
\drawArrowShift{f}{0,-1}
\drawArrowShift{B}{0,-1}
\bracketCup{b}{b2}

\drawEndNodes{
    f/$A$,
    B/$B$
}
\end{tikzpicture}


==> ClosedDiags/StringGen/4a.tex <==
\tikzsetnextfilename{ClosedDiags/StringGen/4a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A/$X$/0.5,
    B/$Y$/0.5
}

\sShift{A}{0,-1}
\ddShift{B}{0,-1}

\drawEndNodes{
    A/$X$/,
    B/$Y$/
}
\end{tikzpicture}


==> ClosedDiags/StringGen/6.tex <==
\tikzsetnextfilename{ClosedDiags/StringGen/6}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//0
}

\bShift{b1}{0,-1}[right]
\udShift{A}{0,-1}
\ddShift{B}{0,-1}
\bShift{b2}{0,-1}

\drawEndNodes{
    A/
}
\end{tikzpicture}


==> ClosedDiags/StringGen/7.tex <==
\tikzsetnextfilename{ClosedDiags/StringGen/7}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    B/$X$/0.5,
    A/$Y$/0.5,
    b2//0.5,
    C/$Z$/0
}
\ubShift{b1}{0,-1}
\udShift{A}{0,-1}
\ddShift{B}{0,-1}
\udShift{C}{0,-1}
\ubShift{b2}{0,-1}[right]
\drawEndNodes{
    B/$X$/0.5,
    A/$Y$/0.5,
    b2//0.5,
    C/$Z$/0
}
\end{tikzpicture}


==> ClosedDiags/StringGen/down2.tex <==
\tikzsetnextfilename{ClosedDiags/StringGen/down2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A//0
}

\dShift{A}{0,-1}
\drawEndNodes{
    A/
}
\end{tikzpicture}


==> ClosedDiags/StringGen/down5.tex <==
\tikzsetnextfilename{ClosedDiags/StringGen/down5}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//0
}
\bShift{b1}{0,-1}[right]
\udShift{A}{0,-1}
\ddShift{B}{0,-1}
\bShift{b2}{0,-1}
\drawEndNodes{
    A/
}
\end{tikzpicture}


==> ClosedDiags/StringGen/up2.tex <==
\tikzsetnextfilename{ClosedDiags/StringGen/up2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    A//0
}

\uShift{A}{0,-1}
\drawEndNodes{
    A/
}
\end{tikzpicture}


==> ClosedDiags/Sugar/cupCrossing1.tex <==
\tikzsetnextfilename{ClosedDiags/Sugar/cupCrossing1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    Y/$Y$/0.5,
    b2//0.5,
    X/$X$/0.5,
    b3//0.5,
    Z/$Z$/0.5,
    b4//0
}

\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{X}{0,-1}
\sShift{Y}{0,-1}
\sShift{Z}{0,-1}

\bCup{b2}{b3}

\drawEndNodes{
    Y/$Y$/,
    X/$X$/,
    Z/$Z$/
}

\end{tikzpicture}


==> ClosedDiags/Sugar/cupCrossing2.tex <==
\tikzsetnextfilename{ClosedDiags/Sugar/cupCrossing2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    Y/$Y$/0.5,
    b2//0.75,
    X/$X$/0.75,
    b3//0.5,
    Z/$Z$/0.5,
    b4//0
}

\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}


\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}

\sShift{X}{0,-1}

\coord{X1}{X}{-0.25,0}
\coord{X2}{X}{0.25,0}

\coord{X11}{X}{-0.25,0}
\coord{X21}{X}{0.25,0}


\udShift{X1}{-0.5,-1}
\ddShift{X2}{0,-1}
\ddShift{X2}{0,-1}

\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}
\bCup{b2}{b3}

\bead{X11}{X21}{\nu}

\udShift{X1}{0,-1}

\midway{X}{X1}{X2}

\sShift{X}{0,-1}

\bead{X1}{X2}{\nu^{-1}}

\drawEndNodes{
    Y/$Y$/,
    X/$X$/,
    Z/$Z$/
}

\end{tikzpicture}


==> ClosedDiags/Sugar/cupCrossing3.tex <==
\tikzsetnextfilename{ClosedDiags/Sugar/cupCrossing3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    Y//0.5,
    b2//0.75,
    X/$X$/0.75,
    b3//0.5,
    Z//0.5,
    b4//0
}

\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}


\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}

\sShift{X}{0,-1}

\coord{X1}{X}{-0.25,0}
\coord{X2}{X}{0.25,0}

\coord{X11}{X}{-0.25,0}
\coord{X21}{X}{0.25,0}


\udShift{X1}{-0.5,-1}
\ddShift{X2}{0,-1}
\ddShift{X2}{0.5,-1}

\bShift{b2}{0.5,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b3}{-0.5,-1}
\bCup{b2}{b3}[0.25]

\bead{X11}{X21}{\nu}

\udShift{X1}{0,-1}
\udShift{X1}{0,-1}
\ddShift{X2}{0,-1}

\midway{X}{X1}{X2}

\sShift{X}{0,-1}

\bead{X1}{X2}{\nu^{-1}}

\end{tikzpicture}


==> ClosedDiags/Sugar/cupCrossing3a.tex <==
\tikzsetnextfilename{ClosedDiags/Sugar/cupCrossing3a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    Y//0.5,
    b2//0.75,
    X/$X$/0.75,
    b3//0.5,
    Z//0.5,
    b4//0
}

\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b1}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Y}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}
\sShift{Z}{0,-1}


\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}

\sShift{X}{0,-1}

\coord{X1}{X}{-0.25,0}
\coord{X2}{X}{0.25,0}

\coord{X11}{X}{-0.25,0}
\coord{X21}{X}{0.25,0}


\udShift{X1}{-0.5,-1}
\ddShift{X2}{0,-1}
\ddShift{X2}{0.5,-1}

\bShift{b2}{0.5,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b3}{-0.5,-1}
\bCup{b2}{b3}[0.25]

\bead{X11}{X21}{\nu}

\udShift{X1}{0,-1}
\udShift{X1}{0,-1}
\ddShift{X2}{0,-1}

\midway{X}{X1}{X2}

\sShift{X}{0,-1}

\bead{X1}{X2}{\nu^{-1}}

\end{tikzpicture}


==> ClosedDiags/WellDef/cap/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cap/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/2.5,
    B/{$B$}/0.5,
    b4//0
}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coord{b3}{B}{-0.5,0}
\coord{C2}{B}{-1,0}
\coord{C1}{A}{1,0}
\coord{b2}{A}{0.5,0}

\ddCap{C1}{C2}[0.25]
\bCap{b2}{b3}[0.75]

\udShift{C1}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\sShift{B}{0,-1}
\sShift{B}{0,-1}

\ddShift{C2}{0,-1}
\ddShift{C2}{0,-1}

\udShift{C1}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}

\bCup{b2}{b3}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\drawEndNodes{
    A/{$A$},
    C1/{$C$},
    C2/{$C$},
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cap/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cap/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/3.5,
    B/{$B$}/0.5,
    b4//0
}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coordinate[shift={(-0.5,0)}] (b3) at (B);
\coordinate[shift={(-1,0)}] (C2) at (B);
\coordinate[shift={(-1.5,0)}] (C1) at (B);
\coordinate[shift={(-2,0)}] (b2) at (B);

\ddCap{C1}{C2}[0.25]
\bCap{b2}{b3}[0.75]

\coordinate[shift={(-1,0)}] (C0) at (C1);
\coordinate[shift={(-1.5,0)}] (C00) at (C1);

\ddCup{C0}{C1}
\ddCap{C00}{C0}[0.25]

\bShift{b2}{0,-0.75}[right]
\bShift{b3}{0,-0.75}

\sShift{B}{0,-1}
\sShift{B}{0,-1}

\ddShift{C2}{0,-1}
\ddShift{C2}{0,-1}

\sShift{A}{0,-1}
\sShift{A}{0,-1}

\bCup{b2}{b3}[0.75]

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{C00}{0,-1}
\udShift{C00}{0,-1}

\drawEndNodes{
    A/{$A$},
    C2/{$C$},
    C00/{$C$},
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cap/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cap/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/2.5,
    B/{$B$}/0.5,
    b4//0
}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coordinate[shift={(-0.5,0)}] (b3) at (B);
\coordinate[shift={(-1,0)}] (b2) at (B);

\bCap{b2}{b3}[0.25]

\coordinate[shift={(-1.5,0)}] (C0) at (B);
\coordinate[shift={(-2,0)}] (C00) at (B);

\ddCap{C00}{C0}[0.25]

\ddShift{C0}{0.5,-1}

\bShift{b2}{-0.5,-1}[right]
\bShift{b3}{0,-1}

\sShift{B}{0,-1}
\sShift{B}{0,-1}


\sShift{A}{0,-1}
\sShift{A}{0,-1}

\ddShift{C0}{0,-1}

\bCup{b2}{b3}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{C00}{0,-1}
\udShift{C00}{0,-1}

\drawEndNodes{
    A/{$A$},
    C0/{$C$},
    C00/{$C$},
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cup/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cup/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$X$}/0.5,
    b/{}/0.5,
    A1/{$X$}/0.5,
    B/{$Y$}/0.5,
    C/{$Z$}/0.5,
    b1//0.5
}

\bShift{b}{0,-1}[right]
\bShift{b1}{0,-1}
\ddShift{A}{0,-1}
\udShift{A1}{0,-1}
\udShift{B}{0,-1}
\ddShift{C}{0,-1}

\bShift{b}{0,-1}[right]
\bShift{b1}{0,-1}
\ddShift{A}{0,-1}
\udShift{A1}{0,-1}
\udShift{B}{0,-1}
\ddShift{C}{0,-1}

\coordinate[shift={(-0.5,0)}] (b0) at (A);
\coordinate[shift={(0.5,0)}] (b2) at (b1);

\bCap{b0}{b2}[1]

\ddCup{A}{A1}


\drawBracketShift{b}{0,-1}[right]
\drawBracketShift{b1}{0,-1}
\ddShift{C}{0,-1}

\ddShift{C}{0,-1}
\udShift{B}{-0.5,-1}
\udShift{B}{-0.5,-1}

\bShift{b}{0.5,-1}[right]
\bShift{b1}{0,-1}

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b2}{0,-1}
\bShift{b2}{0,-1}

\udShift{B}{0,-1}
\ddShift{C}{0,-1}
\bCup{b}{b1}

\bShift{b0}{0,-1}[right]
\bShift{b2}{0,-1}

\drawEndNodes{
    B/$Y$,
    C/$Z$
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cup/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cup/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$X$}/0.5,
    b/{}/0.5,
    A1/{$X$}/0.5,
    B/{$Y$}/0.5,
    C/{$Z$}/0.5,
    b1//0.5
}

\bShift{b}{0,-1}[right]
\bShift{b1}{0,-1}
\ddShift{A}{0,-1}
\udShift{A1}{0,-1}
\udShift{B}{0,-1}
\ddShift{C}{0,-1}

\bShift{b}{0,-1}[right]
\bShift{b1}{0,-1}
\ddShift{A}{0,-1}
\udShift{A1}{0,-1}
\udShift{B}{0,-1}
\ddShift{C}{0,-1}

\coordinate[shift={(0,-2)}] (b0) at (A);
\coordinate[shift={(0.5,-2)}] (b2) at (b1);

\bCap{b0}{b2}[1]

\ddCup{A}{A1}


\drawBracketShift{b}{0,-1}[right]
\drawBracketShift{b1}{0,-1}
\ddShift{C}{0,-1}

\ddShift{C}{0,-1}
\udShift{B}{-0.5,-1}
\udShift{B}{-0.5,-1}

\bShift{b}{0.5,-1}[right]
\bShift{b1}{0,-1}

\bShift{b0}{0,-1}[right]
\bShift{b2}{0,-1}

\udShift{B}{0,-1}
\ddShift{C}{0,-1}
\bCup{b}{b1}


\drawEndNodes{
    B/$Y$,
    C/$Z$
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cup2/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cup2/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b0}{b1}{-0.5,-2}
\coord{b5}{b4}{0.5,-2}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddShift{B}{1,-1}
\udShift{C}{0,-1}
\udShift{C}{0,-1}

\ddCup{B}{C}

\bCup{b1}{b2}

\bCap{b0}{b5}[1.5]

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}

\bCup{b3}{b4}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cup2/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cup2/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//2,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b0}{b1}{-0.5,-2}
\coord{b5}{b4}{0.5,-2}


\coord{bMid1}{b0}{2.5,0}
\coord{bMid2}{b5}{-2.5,0}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddShift{B}{2,-1}
\udShift{C}{0,-1}
\udShift{C}{0,-1}

\ddCup{B}{C}

\bCup{b1}{b2}

\bCap{b0}{bMid1}[1]
\bCap{bMid2}{b5}[1]
\bbCup{bMid1}{bMid2}

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}

\bCup{b3}{b4}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cup2/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cup2/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1.5,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b5}{b4}{0.5,-2}

\coord{bMid1}{b2}{0,-2}
\coord{bMid2}{b5}{-2.5,0}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddShift{B}{1.5,-1}
\udShift{C}{0,-1}
\udShift{C}{0,-1}

\ddCup{B}{C}


\bCap{bMid2}{b5}[1]
\bbCup{bMid1}{bMid2}

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bCup{b3}{b4}
\bbCup{bMid1}{bMid2}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef/cup2/4.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/cup2/4}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1.5,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b5}{b4}{0.5,-2}

\coord{bMid1}{b2}{0,-2}
\coord{bMid2}{b5}{-2.5,0}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}


\sShift{A}{0,-1}
\udShift{C}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddCup{B}{C}[1]


\bCap{bMid2}{b5}[1]
\bbCup{bMid1}{bMid2}

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bCup{b3}{b4}
\bbCup{bMid1}{bMid2}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef/downEnter/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/downEnter/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    X/$X$/0.5,
    b1//0.5,
    X1//0.5
    X2//0.5
}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\coordinate[shift={(-0.5,0)}] (b0) at (b1);
\coordinate[shift={(0.5,0)}] (b5) at (b4);

\bCap{b0}{b5}[1.5]

\udShift{C}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bCup{b2}{b3}

\udShift{A}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{B}{0,-1}
\udShift{B}{0,-1}

\udShift{A}{0,-1}
\udShift{C}{0,-1}

\bShift{b1}{0,-1}[right]
\drawEndNodes{
    A/{$A$},
    B/{$B$},
    C/{$C$},
    D/{$D$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef/upEnter/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/upEnter/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$X$}/0.5,
    B/{$Y$}/0.5,
    b2//0.5,
    C/{$W$}/0.5,
    D/{$Z$}/0.5,
    b3//0.5,
    b4//0.5
}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}



\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}

\coordinate[shift={(-0.5,-1)}] (b0) at (b1);
\coordinate[shift={(0.5,-1)}] (b5) at (b4);

\udShift{C}{0,-1}
\bShift{b2}{0,-1}[right]

\udShift{C}{0,-1}
\bShift{b2}{0,-1}[right]

\bCap{b0}{b5}[1.7]


\udShift{C}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bCup{b2}{b3}

\udShift{A}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{B}{0,-1}
\udShift{B}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]


\udShift{A}{0,-1}
\udShift{C}{0,-1}

\bCup{b1}{b4}[1]

\coordinate[shift={(0,-2.5)}] (b1) at (b4);
\coordinate[shift={(0,-2.5)}] (b1) at (b4);

\bShift{b1}{0,-1}

\drawEndNodes{
    A/{$X$},
    B/{$Y$},
    C/{$Z$},
    D/{$W$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef/upEnter/2a.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/upEnter/2a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/0.5,
    B/{$B$}/0.5,
    b2//0.5,
    C/{$C$}/0.5,
    D/{$D$}/0.5,
    b3//0.5,
    b4//0
}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\udShift{A}{-0.5,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0.5,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\coordinate[shift={(-1,0)}] (b0) at (b1);
\coordinate[shift={(0.5,0)}] (b5) at (b4);

\bCap{b0}{b5}[1.5]

\udShift{C}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bCup{b2}{b3}

\udShift{A}{0,-1}

\udShift{B}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{B}{0.5,-1}

\udShift{A}{0,-1}
\udShift{C}{0,-1}

\bShift{b1}{-0.5,-1}[right]


\drawEndNodes{
    A/{$A$},
    B/{$B$},
    C/{$C$},
    D/{$D$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef/upEnter/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/upEnter/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/0.5,
    B/{$B$}/1,
    b2//0.5,
    C/{$C$}/0.5,
    D/{$D$}/0.5,
    b3//1,
    b4//0
}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\udShift{C}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bCup{b2}{b3}

\udShift{A}{0,-1}

\udShift{B}{0,-1}
\bShift{b1}{0,-1}[right]


\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{B}{0.5,-1}

\udShift{A}{0,-1}
\udShift{C}{0,-1}

\bShift{b1}{0,-1}[right]

\coordinate[shift={(-0.5,1)}] (b0) at (C);
\coordinate[shift={(1,1)}] (b5) at (D);

\bCap{b0}{b5}[1]

\bShift{b0}{-0.5,-1}[right]
\bShift{b5}{0,-1}

\drawEndNodes{
    A/{$A$},
    B/{$B$},
    C/{$C$},
    D/{$D$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef/upLeaveLeft/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/upLeaveLeft/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$X$}/0.5,
    b2//0.5,
    B/{$Y$}/0.5,
    C/{$Z$}/0.5,
    D/{$W$}/0.5,
    b3//0.5,
    E/{$U$}/0.5,
    b4//0.5
}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\udShift{C}{0,-1.5}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\udShift{C}{0,-1.5}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\coordinate[shift={(-0.5,0)}] (A1) at (b1);
\coordinate[shift={(-2,0)}] (A2) at (b1);

\coordinate[shift={(-1,0)}] (B1) at (b1);
\coordinate[shift={(-1.5,0)}] (B2) at (b1);

\coordinate[shift={(-0.5,0)}] (b0) at (A2);
\coordinate[shift={(0.5,0)}] (b5) at (b4);

\bracketCap{b0}{b5}[1.5]

\ddCap{A2}{A1}[.75]
\ddCup{A1}{A}

\ddCap{B2}{B1}[0.25]

\ddShift{B1}{0,-1}
\ddShift{B1}{1.5,-1.5}

\udShift{B}{0,-1.5}
\udShift{C}{0,-1.5}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1}[right]
\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}
\drawBracketShift{b4}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}


\udShift{B}{0,-1}
\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\bracketCup{b1}{b4}[1]

\ddCup{B1}{B}

\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\udShift{B2}{0,-1.5}
\udShift{B2}{0,-1}
\udShift{B2}{0,-1}

\udShift{A2}{0,-1.5}
\udShift{A2}{0,-1}
\udShift{A2}{0,-1}

\drawBracketShift{b0}{0,-1.5}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]

\drawBracketShift{b5}{0,-1.5}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}


\drawEndNodes{
    A2/{$X$},
    B2/{$Y$},
    C/{$Z$},
    D/{$W$},
    E/{$U$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef/upLeaveLeft/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/upLeaveLeft/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$X$}/0.5,
    b2//0.5,
    B/{$Y$}/0.5,
    C/{$Z$}/0.5,
    D/{$W$}/0.5,
    b3//0.5,
    E/{$U$}/0.5,
    b4//0.5
}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\udShift{C}{0,-1.5}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\udShift{A}{0,-1}
\udShift{B}{0,-1}
\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\drawBracketShift{b1}{0,-1}[right]
\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}
\drawBracketShift{b4}{0,-1}

\coordinate[shift={(-0.5,0)}] (b0) at (b1);
\coordinate[shift={(0.5,0)}] (b5) at (b4);

\bracketCap{b0}{b5}[1.5]

\udShift{A}{-0.5,-1}
\drawBracketShift{b1}{0.5,-1}[right]

\udShift{B}{0,-1}
\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}
\drawBracketShift{b4}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}


\udShift{B}{0,-1}
\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\bracketCup{b1}{b4}[1]

\drawBracketShift{b2}{0.5,-1}[right]
\drawBracketShift{b3}{0,-1}

\udShift{B}{-0.5,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]

\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}

\udShift{A}{0,-1}
\udShift{A}{0,-1}
\udShift{B}{0,-1}
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}

\udShift{A}{0,-1}

\drawEndNodes{
    A/{$X$},
    B/{$Y$},
    C/{$Z$},
    D/{$W$},
    E/{$U$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef/upLeaveLeft/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef/upLeaveLeft/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$X$}/0.5,
    b2//0.5,
    B/{$Y$}/0.5,
    C/{$Z$}/0.5,
    D/{$W$}/0.5,
    b3//0.5,
    E/{$U$}/0.5,
    b4//0.5
}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\ddShift{C}{0,-1.5}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\ddShift{C}{0,-1.5}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\coordinate[shift={(0,0)}] (b0) at (b1);
\coordinate[shift={(0,0)}] (b5) at (b4);

\udShift{A}{0,-1}
\drawBracketShift{b1}{0,-1}[right]

\udShift{B}{0,-1}
\ddShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}
\drawBracketShift{b4}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}


\udShift{B}{0,-1}
\ddShift{C}{0,-1}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}

\bracketCup{b1}{b4}[1]

\drawBracketShift{b2}{0.5,-1}[right]
\drawBracketShift{b3}{0,-1}

\udShift{B}{-0.5,-1}

\ddShift{C}{0,-1}
\ddShift{C}{0,-1.5}
\ddShift{D}{0,-1}
\ddShift{E}{0,-1}
\ddShift{D}{0,-1.5}
\ddShift{E}{0,-1.5}

\bracketCup{b2}{b3}[0.75]

\drawBracketShift{b0}{0,-1.5}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]

\drawBracketShift{b5}{0,-1.5}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}

\udShift{A}{0,-1.5}
\udShift{A}{0,-1}
\udShift{A}{0,-1}

\udShift{B}{0,-1.5}

\drawEndNodes{
    A/{$X$},
    B/{$Y$},
    C/{$Z$},
    D/{$W$},
    E/{$U$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef2/cap/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cap/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/2.5,
    B/{$B$}/0.5,
    b4//0
}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coord{b3}{B}{-0.5,0}
\coord{C2}{B}{-1,0}
\coord{C1}{A}{1,0}
\coord{b2}{A}{0.5,0}

\ddCap{C1}{C2}[0.25]
\bCap{b2}{b3}[0.75]

\udShift{C1}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\sShift{B}{0,-1}
\sShift{B}{0,-1}

\ddShift{C2}{0,-1}
\ddShift{C2}{0,-1}

\udShift{C1}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}

\bCup{b2}{b3}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\drawEndNodes{
    A/{$A$},
    C1/{$C$},
    C2/{$C$},
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cap/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cap/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/3.5,
    B/{$B$}/0.5,
    b4//0
}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coordinate[shift={(-0.5,0)}] (b3) at (B);
\coordinate[shift={(-1,0)}] (C2) at (B);
\coordinate[shift={(-1.5,0)}] (C1) at (B);
\coordinate[shift={(-2,0)}] (b2) at (B);

\ddCap{C1}{C2}[0.25]
\bCap{b2}{b3}[0.75]

\coordinate[shift={(-1,0)}] (C0) at (C1);
\coordinate[shift={(-1.5,0)}] (C00) at (C1);

\ddCup{C0}{C1}
\ddCap{C00}{C0}[0.25]

\bShift{b2}{0,-0.75}[right]
\bShift{b3}{0,-0.75}

\sShift{B}{0,-1}
\sShift{B}{0,-1}

\ddShift{C2}{0,-1}
\ddShift{C2}{0,-1}

\sShift{A}{0,-1}
\sShift{A}{0,-1}

\bCup{b2}{b3}[0.75]

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{C00}{0,-1}
\udShift{C00}{0,-1}

\drawEndNodes{
    A/{$A$},
    C2/{$C$},
    C00/{$C$},
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cap/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cap/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/2.5,
    B/{$B$}/0.5,
    b4//0
}

\sShift{A}{0,-1}
\sShift{B}{0,-1}

\coordinate[shift={(-0.5,0)}] (b3) at (B);
\coordinate[shift={(-1,0)}] (b2) at (B);

\bCap{b2}{b3}[0.25]

\coordinate[shift={(-1.5,0)}] (C0) at (B);
\coordinate[shift={(-2,0)}] (C00) at (B);

\ddCap{C00}{C0}[0.25]

\ddShift{C0}{0.5,-1}

\bShift{b2}{-0.5,-1}[right]
\bShift{b3}{0,-1}

\sShift{B}{0,-1}
\sShift{B}{0,-1}


\sShift{A}{0,-1}
\sShift{A}{0,-1}

\ddShift{C0}{0,-1}

\bCup{b2}{b3}

\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{C00}{0,-1}
\udShift{C00}{0,-1}

\drawEndNodes{
    A/{$A$},
    C0/{$C$},
    C00/{$C$},
    B/{$B$}
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cup/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cup/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$X$}/0.5,
    b/{}/0.5,
    A1/{$X$}/0.75,
    B/{$Y$}/0.75,
    b1//0.5
}

\bShift{b}{0,-1}[right]
\bShift{b1}{0,-1}
\ddShift{A}{0,-1}
\udShift{A1}{0,-1}
\sShift{B}{0,-1}

\bShift{b}{0,-1}[right]
\bShift{b1}{0,-1}
\ddShift{A}{0,-1}
\udShift{A1}{0,-1}
\sShift{B}{0,-1}

\coord{Y1}{B}{-0.25,0}
\coord{Y2}{B}{0.25,0}

\coordinate[shift={(-0.5,0)}] (B1) at (A);
\coordinate[shift={(-0.5,0)}] (B2) at (B1);
\coordinate[shift={(-0.5,0)}] (b0) at (B2);
\coordinate[shift={(0.5,0)}] (b2) at (b1);

\ddCap{B2}{B1}[0.25]
\bCap{b0}{b2}[1]

\ddCup{A}{A1}
\ddCup{B1}{Y1}[1]

\drawBracketShift{b}{0,-1}[right]
\drawBracketShift{b1}{0,-1}
\udShift{B2}{0,-1}

\udShift{B2}{0,-1}
\bCup{b}{b1}

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b2}{0,-1}
\bShift{b2}{0,-1}

\bead{Y1}{Y2}{\nu}


\drawEndNodes{
    B2/$B$
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cup2/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cup2/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b0}{b1}{-0.5,-2}
\coord{b5}{b4}{0.5,-2}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddShift{B}{1,-1}
\udShift{C}{0,-1}
\udShift{C}{0,-1}

\ddCup{B}{C}

\bCup{b1}{b2}

\bCap{b0}{b5}[1.5]

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}

\bCup{b3}{b4}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cup2/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cup2/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//2,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b0}{b1}{-0.5,-2}
\coord{b5}{b4}{0.5,-2}


\coord{bMid1}{b0}{2.5,0}
\coord{bMid2}{b5}{-2.5,0}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddShift{B}{2,-1}
\udShift{C}{0,-1}
\udShift{C}{0,-1}

\ddCup{B}{C}

\bCup{b1}{b2}

\bCap{b0}{bMid1}[1]
\bCap{bMid2}{b5}[1]
\bbCup{bMid1}{bMid2}

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}
\bShift{b0}{0,-1}[right]
\bShift{b5}{0,-1}

\bCup{b3}{b4}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cup2/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cup2/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1.5,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b5}{b4}{0.5,-2}

\coord{bMid1}{b2}{0,-2}
\coord{bMid2}{b5}{-2.5,0}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddShift{B}{1.5,-1}
\udShift{C}{0,-1}
\udShift{C}{0,-1}

\ddCup{B}{C}


\bCap{bMid2}{b5}[1]
\bbCup{bMid1}{bMid2}

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}
\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bCup{b3}{b4}
\bbCup{bMid1}{bMid2}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/cup2/4.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/cup2/4}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    B//0.5,
    b2//1.5,
    b3//0.5,
    C//0.5,
    D//0.5,
    b4//0
}

\coord{b5}{b4}{0.5,-2}

\coord{bMid1}{b2}{0,-2}
\coord{bMid2}{b5}{-2.5,0}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}


\sShift{A}{0,-1}
\udShift{C}{-0,-1}
\udShift{C}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}
\sShift{D}{0,-1}

\sShift{A}{0,-1}
\ddShift{B}{-0,-1}

\ddCup{B}{C}[1]


\bCap{bMid2}{b5}[1]
\bbCup{bMid1}{bMid2}

\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{A}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}
\sShift{D}{0,-1}


\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]
\bShift{b1}{0,-1}[right]

\bShift{b3}{0,-1}[right]
\bShift{b4}{0,-1}

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bCup{b3}{b4}
\bbCup{bMid1}{bMid2}


\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/WellDef2/upEnter/1.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/upEnter/1}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/0.5,
    B/{$B$}/0.5,
    b2//0.5,
    C/{$C$}/0.5,
    D/{$D$}/0.5,
    b3//0.5,
    b4//0
}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}

\coordinate[shift={(-0.5,0)}] (b0) at (b1);
\coordinate[shift={(0.5,0)}] (b5) at (b4);

\bCap{b0}{b5}[1.5]

\udShift{C}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bCup{b2}{b3}

\udShift{A}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{B}{0,-1}
\udShift{B}{0,-1}

\udShift{A}{0,-1}
\udShift{C}{0,-1}

\bShift{b1}{0,-1}[right]
\drawEndNodes{
    A/{$A$},
    B/{$B$},
    C/{$C$},
    D/{$D$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef2/upEnter/2.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/upEnter/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/0.5,
    B/{$B$}/0.5,
    b2//0.5,
    C/{$C$}/0.5,
    D/{$D$}/0.5,
    b3//0.5,
    b4//0.5
}

\udShift{A}{0,-1}
\udShift{B}{0,-1}

\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b1}{0,-1}[right]
\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}
\bShift{b4}{0,-1}



\udShift{C}{0,-1}
\ddShift{D}{0,-1}

\bShift{b2}{0,-1}[right]
\bShift{b3}{0,-1}

\coordinate[shift={(-0.5,-1)}] (b0) at (b1);
\coordinate[shift={(0.5,-1)}] (b5) at (b4);

\udShift{C}{0,-1}
\bShift{b2}{0,-1}[right]

\udShift{C}{0,-1}
\bShift{b2}{0,-1}[right]

\bCap{b0}{b5}[1.7]


\udShift{C}{-0.5,-1}
\bShift{b2}{0.5,-1}[right]
\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bShift{b3}{0,-1}

\ddShift{D}{0,-1}
\ddShift{D}{0,-1}

\bCup{b2}{b3}

\udShift{A}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]

\bShift{b0}{0,-1}[right]
\bShift{b0}{0,-1}[right]

\bShift{b5}{0,-1}
\bShift{b5}{0,-1}

\bShift{b4}{0,-1}
\bShift{b4}{0,-1}

\udShift{B}{0,-1}
\udShift{B}{-0.5,-1}
\bShift{b1}{0.5,-1}[right]


\udShift{A}{0,-1}
\udShift{C}{0,-1}

\bCup{b1}{b4}[1]

\coordinate[shift={(0,-2.5)}] (b1) at (b4);
\coordinate[shift={(0,-2.5)}] (b1) at (b4);

\bShift{b1}{0,-1}

\drawEndNodes{
    A/{$A$},
    B/{$B$},
    C/{$C$},
    D/{$D$}
}

\end{tikzpicture}


==> ClosedDiags/WellDef2/upLeaveLeft/3.tex <==
\tikzsetnextfilename{ClosedDiags/WellDef2/upLeaveLeft/3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    A/{$A$}/0.5,
    b2//0.5,
    B/{$B$}/0.5,
    C/{$C$}/0.5,
    b3//0.5,
    E/{$E$}/0.5,
    b4//0.5
}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\sShift{C}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\udShift{A}{0,-1.5}
\udShift{B}{0,-1.5}
\sShift{C}{0,-1.5}
\ddShift{E}{0,-1.5}

\drawBracketShift{b1}{0,-1.5}[right]
\drawBracketShift{b2}{0,-1.5}[right]
\drawBracketShift{b3}{0,-1.5}
\drawBracketShift{b4}{0,-1.5}

\coordinate[shift={(0,0)}] (b0) at (b1);
\coordinate[shift={(0,0)}] (b5) at (b4);

\udShift{A}{0,-1}
\drawBracketShift{b1}{0,-1}[right]

\udShift{B}{0,-1}
\sShift{C}{0,-1}
\ddShift{E}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}
\drawBracketShift{b4}{0,-1}

\drawBracketShift{b2}{0,-1}[right]
\drawBracketShift{b3}{0,-1}


\udShift{B}{0,-1}
\sShift{C}{0,-1}
\ddShift{E}{0,-1}

\bracketCup{b1}{b4}[1]

\drawBracketShift{b2}{0.5,-1}[right]
\drawBracketShift{b3}{0,-1}

\udShift{B}{-0.5,-1}

\sShift{C}{0,-1}
\sShift{C}{0,-1.5}
\ddShift{E}{0,-1}
\ddShift{E}{0,-1.5}

\bracketCup{b2}{b3}[0.75]

\drawBracketShift{b0}{0,-1.5}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]
\drawBracketShift{b0}{0,-1}[right]

\drawBracketShift{b5}{0,-1.5}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}
\drawBracketShift{b5}{0,-1}

\udShift{A}{0,-1.5}
\udShift{A}{0,-1}
\udShift{A}{0,-1}

\udShift{B}{0,-1.5}

\drawEndNodes{
    A/{$A$},
    B/{$B$},
    C/{$C$},
    E/{$E$}
}

\end{tikzpicture}


==> ClosedDiags/XReflectedGen/11a.tex <==
\tikzsetnextfilename{ClosedDiags/XReflectedGen/11a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}

\XbbCup{b1}{b2}
\coord{b1}{b1}{0,-1}

\drawEndNodes{b1/}

\end{tikzpicture}


==> ClosedDiags/XYReflectedGen/11.tex <==
\tikzsetnextfilename{ClosedDiags/XYReflectedGen/11}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}

\ddShift{A}{0,-1}
\bCup{b1}{b2}

\drawEndNodes{
    A//
}
\end{tikzpicture}


==> ClosedDiags/XYReflectedGen/12a.tex <==
\tikzsetnextfilename{ClosedDiags/XYReflectedGen/12a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1]
\drawStartNodes{
    b1//0.5,
    A//0.5,
    b2//0
}
\coordinate[shift={(0,-1)}] (b1) at (b1);
\coordinate[shift={(0,-1)}] (b2) at (b2);
\XbbCap{b1}{b2}

\drawEndNodes{b1/}

\end{tikzpicture}


==> ClosedDiags/XYReflectedGen/2.tex <==
\tikzsetnextfilename{ClosedDiags/XYReflectedGen/2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    B//0.5,
    b2//0.5,
    A//0
}

\bShift{b1}{0,-1}[right]
\sShift{B}{0,-1}
\ddShift{A}{-0.5,-1}
\bShift{b2}{0.5,-1}

\drawEndNodes{
    A//,
    B//
}

\end{tikzpicture}


==> ClosedDiags/XYReflectedGen/2a.tex <==
\tikzsetnextfilename{ClosedDiags/XYReflectedGen/2a}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1//0.5,
    B//0.5,
    A//0.5,
    b2//0
}

\bShift{b1}{0,-1}[right]
\ddShift{B}{0,-1}
\ddShift{A}{0.5,-1}
\bShift{b2}{-0.5,-1}

\drawEndNodes{
    A//,
    B//
}

\end{tikzpicture}


==> ClosedDiags/basic2.tex <==
\tikzsetnextfilename{ClosedDiags/basic2}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    A/{$A$}/0
}
\upArrowShift{A}{0,-1}


\drawEndNodes{
    A/{$A$}
}

\end{tikzpicture}


==> ClosedDiags/basic3.tex <==
\tikzsetnextfilename{ClosedDiags/basic3}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1/{}/0.5,
    A/{$A$}/0.5,
    B/{$B$}/0.5,
    b2/{}/0
}
\drawBracketShift{b1}{0,-1}[right]
\drawArrowShift{A}{0,-1}
\upArrowShift{B}{0,-1}
\drawBracketShift{b2}{0,-1}

\drawEndNodes{
    A/{$A$},
    B/{$B$}
}

\end{tikzpicture}


==> ClosedDiags/invbasic4.tex <==
\tikzsetnextfilename{ClosedDiags/invbasic4}
\begin{tikzpicture}[baseline={(current bounding box.center)}, xscale=1
]
\drawStartNodes{
    b1/{}/0.5,
    B/{$B$}/0.5,
    C/{$C$}/0.5,
    b2/{}/0
}
\drawBracketShift{b1}{0,-1}[right]
\drawArrowShift{B}{0,-1}
\drawArrowShift{C}{0.5,-1}
\drawBracketShift{b2}{-0.5,-1}

\drawEndNodes{
    B/{$B$},
    C/{$C$}
}

\end{tikzpicture}


==> clipMacros.tex <==
\setsepchar[.]{;./}

\xdef\gapWidth{1.2}
\xdef\hlWidth{1.2}
\xdef\lineWidth{0.4}
\xdef\outerLineWidth{0.2}


\tikzmath{
    function angle(\a){
        return Mod(\a,360);
    };
    function bisect(\i,\o){
        if angle(\i)<angle(\o) then{
            return angle((angle(\i)+angle(\o))/2);
        }
        else{
            return angle(((angle(\i)+angle(\o))/2)-180);
        };
    };
    function shiftToFactor(\s,\x1,\x2){
        if \x1==\x2 then{
            return 0;
        } else{
            return (1+(\s/(\x1-\x2)))/(28.45274);
        };
    };
    function vecAngle(\x,\y){
        if \y<0 then {
            \s=-1;
        } else {
            \s=1;
        };
        return 180+\s*acos(\x/(veclen(\x,\y)));
    };
    function hlDblSep(\n){
        return \lineWidth+2*\gapWidth+2*(\n-1)*(\hlWidth+\gapWidth);
    };
    function hlDblSep2(\n){
        return 2*\outerLineWidth+4*\gapWidth+\lineWidth+2*\gapWidth+2*(\n-1)*(\hlWidth+\gapWidth);
    };
    function TCLShft(\n){
        return ((\lineWidth-hlDblSep(\n))/2)-\hlWidth;
    };
    function TCelShft(\l,\r){
        return (1/2)*(\r-\l)*(\hlWidth+\gapWidth);
    };
    function TCWidth(\n,\l,\r){
        return \n+2*\hlWidth+hlDblSep(\l)+hlDblSep(\r)+10;
    };
    function TCWidthX(\n,\l,\r){
        return \n+(\l+\r)*(\hlWidth+\gapWidth)+10;
    };
    function symWidth(\n,\l,\r){
        return (max(\l*2*(\hlWidth+\gapWidth),\r*2*(\hlWidth+\gapWidth)))+\n;
    };
    function testing(\l,\r){
        return (max(\l*2*(\hlWidth+\gapWidth),\r*2*(\hlWidth+\gapWidth)));
    };
    function twoCellWidth(\n,\l,\r,\n2,\l2,\r2){
        return 10+max(symWidth(\n,\l,\r), symWidth(\n2,\l2,\r2));
    };
    function outerLineSep(\n){
        return \lineWidth+2*\gapWidth+2*\n*(\hlWidth+\gapWidth);
    };
    function joinAngle(\i,\n){
        return 180*(1-(1/(2*\n)))+(1-\i)*(180/\n);
    };
    function spread(\i,\n,\w){
        if \n==1 then{
            return 0;
        }else{
            return (\i-1)*(\w/(\n-1))-(\w/2);
        };
    };
    function idRad(\i){
        return (1/2)*\lineWidth+(1/2)*\hlWidth+\gapWidth+(\i-1)*(\hlWidth+\gapWidth);
    };
}

\newcommand{\ifempty}[2]{
    \ifthenelse{\equal{}{#1}}{
        #2
    }{}
}

\newcommand{\ifnonempty}[2]{
    \ifthenelse{\equal{}{#1}}{}{
        #2
    }
}

\newcommandx{\place}[4][3=0]{
    \coordinate[shift={(#2,#3)}] (tempPlace) at (#4); 
    \coordinate (#1) at (tempPlace); 
}

\newcommand{\listLength}[2]{
    \edef\inputLL{#1}
    \xdef#2{0}
    \foreach \i in \inputLL{
        \tikzmath{
            integer \currentLength;
            \currentLength = #2+1;
        }
        \xdef#2{\currentLength}
    }
}

\newcommand{\listLengthX}[2]{
    \edef\inputLLX{#1}
    \xdef#2{0}
    \foreach \i in \inputLLX{
        \ifthenelse{\equal{\i}{}}{}{
            \tikzmath{
                integer \currentLength;
                \currentLength = #2+1;
            }
            \xdef#2{\currentLength}
        }
    }
}

\newcommand{\reverseList}[2]{
    \edef\inputRL{#1}
    \xdef#2{}
    \foreach \x[count=\i] in \inputRL{
        \ifthenelse{\equal{#2}{}}{
            \xdef#2{\x}
        }{
            \xdef#2{\x,#2}
        }
    }
}

\newcommandx{\joinTarget}[5][4=\nodesWidth,5=-1,usedefault]{
    \readlist*\inputJT{#1}
    \xdef\xCoordinateList{}
    \xdef\yCoordinateList{}

    \foreachitem \n \in \inputJT{
        \gettikzxy{(\n)}{\ax}{\ay}
        \xdef\xCoordinateList{\ax,\xCoordinateList}
        \xdef\yCoordinateList{\ay,\yCoordinateList}
    }
    \tikzmath{
        \minX=min(\xCoordinateList);
        \maxX=max(\xCoordinateList);
        \xCoordinate=(\maxX+\minX)/2;
        \minY=min(\yCoordinateList);
        \maxY=max(\yCoordinateList);
        \width=\maxX-\minX;
    }
    \ifdim #5 pt < 0 pt
        \xdef\yCoordinate{\minY}
    \else
        \xdef\yCoordinate{\maxY}
    \fi{}
    \xdef#4{\width}
    \coordinate[shift={(0,#2)}] (#3) at (\xCoordinate pt, \yCoordinate pt);
}

\newcommandx{\splitTargets}[4]{
    \readlist*\splitInput{#2}
    \foreach \i in {1,...,\splitInputlen}{
        \tikzmath{
            \p=spread(\i,\splitInputlen,#3);
        }
        \coordinate[shift={(\p,-#4)}] (\splitInput[\i]) at (#1);
    }
}

\newcommandx{\halfPath}[3][1=]{
    \begin{scope}
        \begin{pgfinterruptboundingbox}
        \clip #2 #3;
        \end{pgfinterruptboundingbox}
        \draw[#1] #2;
    \end{scope}
}

\newcommandx{\removeEmpty}[2]{
    \xdef\removeEmptyInput{#1}
    \xdef\output{}
    \foreach \x[count=\i] in \removeEmptyInput{
        \ifnonempty{\x}{
            \ifnonempty{\output}{
                \xdef\output{\output,\x}
            }
            \ifempty{\output}{
                \xdef\output{\x}
            }
        }
    }
    \xdef#2{\output}
}

\newcommandx{\highlightSide}[4]{
    \removeEmpty{#1}{\coloursI}        
    \listLength{\coloursI}{\colourslenI}
    \removeEmpty{#2}{\coloursII}
    \listLength{\coloursII}{\colourslenII}

    \foreach \c [count=\k] in \coloursI{
        \ifthenelse{\equal{\c}{}}{}{
        \halfPath[
            double,
            double=white,
            draw=\c, 
            double distance=hlDblSep(\colourslenI+\colourslenII+1-\k), 
            line width=\hlWidth pt,
            rounded corners=0.5
        ]{#3}{#4}
        }
    }
    \foreach \c [count=\k] in \coloursII{
        \ifthenelse{\equal{\c}{}}{}{
        \halfPath[
            double,
            double=white,
            draw=\c, 
            double distance=hlDblSep(\colourslenII+1-\k), 
            line width=\hlWidth pt,
            rounded corners=0.5,
            NTDash
            ]{#3}{#4}
        }
    }
}

\newcommandx{\highlight}[7][7=]{
    \xdef\coloursTempI{#2}
    \xdef\coloursTempII{#3}
    \reverseList{#4}{\coloursTempIII}    
    \highlightSide{\coloursTempI}{\coloursTempII}{#1}{#5}
    \highlightSide{\coloursTempI}{\coloursTempIII}{#1}{#6}
    
    \listLengthX{#3}{\ntleftlen}
    \listLengthX{#4}{\ntrightlen}
    \tikzmath{
        integer \nt;
        \nt=\ntleftlen+\ntrightlen;
    }
    \ifnum \nt>0
        \draw[line width=\lineWidth,NTDash,#7] #1;
    \else
        \draw[line width=\lineWidth,#7] #1;
    \fi
}

\newcommandx{\clipS}[4][3=\leftClip,4=\rightClip,usedefault]{
    \gettikzxy{(#1)}{\ix}{\iy}
    \gettikzxy{(#2)}{\ox}{\oy}

    \ifdim \iy>\oy
        \xdef\s{-1}
    \else
        \xdef\s{1}
    \fi

    \ifdim \ix <\ox
        \xdef#3{
            --++(0,\s*3)
            -|($(#1)+(-3,-\s*3)$)
            -|(#1)
        }
        \xdef#4{
            |-++(3,\s*3)
            |-($(#1)+(0,-\s*3)$)
            --(#1)
        }
    \else
        \xdef#3{
            |-++(-3,\s*3)
            |-($(#1)+(0,-\s*3)$)
            --(#1)
        }
        \xdef#4{
            --++(0,\s*3)
            -|($(#1)+(3,-\s*3)$)
            -|(#1)
        }
    \fi{}
}

\newcommandx{\drawS}[6][3=,4=,5=,6=,usedefault]{
    \clipS{#1}{#2}
    \highlight{(#1) to[out=-90, in=90] (#2)}{#3}{#4}{#5}{\leftClip}{\rightClip}[#6]
}

\newcommandx{\strS}[5][3=,4=,5=]{
    \drawS{#1}{#2}[#3][#4][#5]
    \coordinate (#1) at (#2);
}

\newcommandx{\strSX}[5][3=,4=,5=]{
    \coordinate[shift={(#2)}] (temp) at (#1);
    \drawS{#1}{temp}[#3][#4][#5]
    \coordinate (#1) at (temp);
}

\newcommandx{\drawIdTo}[6][3=,4=,5=,6=,usedefault]{
    \clipS{#1}{#2}
    \highlight{(#1)--(#1|-#2)}{#3}{#4}{#5}{\leftClip}{\rightClip}[#6]
}

\newcommandx{\strIdTo}[6][3=,4=,5=,6=,usedefault]{
    \drawIdTo{#1}{#2}[#3][#4][#5][#6]
    \coordinate (#1) at (#1|-#2);
}

\newcommandx{\strId}[6][2=,3=,4=,5=1,6=,usedefault]{
    \coordinate[shift={(0,-#5)}] (temp) at (#1);
    \strIdTo{#1}{temp}[#2][#3][#4][#6]
}


\newcommandx{\strBraid}[9][3=,4=,5=,6=,7=,8=1,9=;,usedefault]{
    \joinTarget{#1;#2}{0}{topLevel}
    \readlist\options{#9}
    \xdef\optionI{\options[1,1]}
    \xdef\optionII{\options[2,1]}

    \coordinate[shift={(0,-#8)}] (rightBottom) at (#2|-topLevel);
    \coordinate[shift={(0,-#8)}] (leftBottom) at (#1|-topLevel);

    \xdef\overPath{
        (#1) to[out=-90, in=90] (rightBottom)
    }

    \clipS{#1}{rightBottom}
    \begin{scope}
        \begin{pgfinterruptboundingbox}
            \clip \overPath\rightClip;
        \end{pgfinterruptboundingbox}
        \drawS{#2}{leftBottom}[#3,#5][#6][#7][\optionII]
    \end{scope}
    \begin{scope}
        \begin{pgfinterruptboundingbox}
            \clip \overPath\leftClip;
        \end{pgfinterruptboundingbox}
        \drawS{#2}{leftBottom}[#3,#4][#6][#7][\optionII]
    \end{scope}
    \drawS{#1}{rightBottom}[white,#3][#4][#5][\optionI]
    \coordinate (#1) at (rightBottom);
    \coordinate (#2) at (leftBottom);
}

\newcommandx{\strBraidX}[3][2=1,3=;,usedefault]{
    \readlist*\braidInput{#1}

    \xdef\topN{\braidInput[1,1]}
    \xdef\topFCol{\braidInput[1,2]}
    \xdef\topNTLCol{\braidInput[1,3]}
    \xdef\topNTRCol{\braidInput[1,4]}
    \xdef\botN{\braidInput[2,1]}
    \xdef\botFCol{\braidInput[2,2]}
    \xdef\botNTLCol{\braidInput[2,3]}
    \xdef\botNTRCol{\braidInput[2,4]}

    \joinTarget{\topN;\botN}{0}{topLevel}
    \readlist*\options{#3}
    \xdef\optionI{\options[1,1]}
    \xdef\optionII{\options[2,1]}

    \coordinate[shift={(0,-#2)}] (rightBottom) at (\botN|-topLevel);
    \coordinate[shift={(0,-#2)}] (leftBottom) at (\topN|-topLevel);

    \xdef\overPath{
        (\topN) to[out=-90, in=90] (rightBottom)
    }

    \clipS{\topN}{rightBottom}
    \begin{scope}
        \begin{pgfinterruptboundingbox}
            \clip \overPath\rightClip;
        \end{pgfinterruptboundingbox}

        \drawS{\botN}{leftBottom}[
            \topFCol,
            \topNTRCol,
            \botFCol
        ][\botNTLCol][\botNTRCol][\optionII]
    \end{scope}
    \begin{scope}
        \begin{pgfinterruptboundingbox}
            \clip \overPath\leftClip;
        \end{pgfinterruptboundingbox}
        \drawS{\botN}{leftBottom}[
            \topFCol,
            \topNTLCol,
            \botFCol
        ][\botNTLCol][\botNTRCol][\optionII]
    \end{scope}
    \drawS{\topN}{rightBottom}[
        white,\topFCol
    ][
        \topNTLCol
    ][
        \topNTRCol][\optionI]
    \coordinate (\topN) at (rightBottom);
    \coordinate (\botN) at (leftBottom);
}

\newcommandx{\drawSCirc}[6][3=,4=,5=,6=-0.5]{
    \joinTarget{#1;#2}{#6}{joinPoint}[][#6]
    \tikzmath{
        \a=sign(#6)*90;
        \shft=(3*(sign(#6)));
    }
    \highlight{
        (#1) to[out=\a, in=180] (joinPoint) to[out=0, in=\a] (#2)
    }{#3}{#4}{#5}{
        |-++(3,-\shft)
        |-($(joinPoint)+(0,\shft)$)
        -|($(#1)+(-3,-\shft)$)
        -|(#1)
    }{
        --++(0,-\shft)
        -|(#1)
    }
}

\newcommandx{\strCup}[6][3=,4=,5=,6=0.5,usedefault]{
    \drawSCirc{#1}{#2}[#3][#4][#5][-#6]
}

\newcommandx{\strCap}[6][3=,4=,5=,6=0.5,usedefault]{
    \drawSCirc{#1}{#2}[#3][#4][#5][#6]
}


\newcommandx{\getNodes}[2]{
    \readlist*\inputGN{#1}
    \xdef\output{}
    \foreach \i in {1,...,\inputGNlen}{
        \ifnum \i=1
            \xdef\output{\inputGN[\i,1]}
        \else
            \xdef\output{\output;\inputGN[\i,1]}
        \fi
    }
    \xdef#2{\output}
}

\newcommandx{\drawFork}[6][1=,2=,4=-0.5,5=-0.5,6=]{
    \getNodes{#3}{\nodes}
    \joinTarget{\nodes}{#4}{join}[][#4]
    \coordinate[shift={(0,#5)}] (exit) at (join);
    
    \readlist*\prong{#3}

    \xdef\natTrans{0}
    \ifnonempty{#2}{
        \xdef\natTrans{1}
    }
    \foreach \i in {1,...,\pronglen}{
        \ifnonempty{prong[\i,1]}{
            \xdef\natTrans{1}
        }
    }
    \ifnum \natTrans>0
        \tikzset{
            temp/.style={
                NTDash,#6,line width=\lineWidth
            }
        }
    \else
        \tikset{
            \temp./style={
                line width=\lineWidth,#6
            }
        }
    \fi

    \tikzmath{
        \s=sign(#4);
        \shft=(-3)*(sign(#4));
    }

    \pgfmathsetmacro\angle{
        -\s*joinAngle(1,\pronglen)
    }

    \clipS{\prong[1,1]}{exit}
    
    \highlightSide{#1}{#2}{
        (\prong[1,1])
        to[out=\s*90,in=\angle] (join) 
        to[out=\s*90, in=-\s*90] (exit)
    }{
        \leftClip
    }

    \draw[temp]      
    (\prong[1,1])
    to[out=\s*90,in=\angle] (join) 
    to[out=\s*90, in=-\s*90] (exit);

    \ifnum \pronglen>1
        \tikzmath{\finish=\pronglen-1;}
        \foreach \i in {1,...,\finish}{

            \xdef\currentNode{\prong[\i,1]}
            \xdef\nextNode{\prong[\i+1,1]}
            \reverseList{\prong[\i,2]}{\currentColours}
            \pgfmathsetmacro\inAngle{
                -\s*joinAngle(\i,\pronglen)
            }
            \pgfmathsetmacro\outAngle{
                -\s*joinAngle(\i+1,\pronglen)
            }
            \highlightSide{#1}{\currentColours}{
                (\currentNode)
                to[out=\s*90,in=\inAngle] (join) 
                to[out=\outAngle, in=\s*90] (\nextNode)
            }{
                --++(0,\shft)
                -|(\currentNode)
            }

            \draw[temp]      
            (\currentNode)
            to[out=\s*90,in=\inAngle] (join) 
            to[out=\outAngle, in=\s*90] (\nextNode);
            
        }
    \fi

    \reverseList{\prong[-1,2]}{\currentColours}

    \pgfmathsetmacro\angle{
        -\s*joinAngle(\pronglen,\pronglen)
    }
    
    \clipS{\prong[-1,1]}{exit}

    \highlightSide{#1}{\currentColours}{
        (\prong[-1,1])
        to[out=\s*90,in=\angle] (join) 
        to[out=\s*90, in=-\s*90] (exit)
    }{\rightClip}

    \draw[temp]         
    (\prong[-1,1])
    to[out=\s*90,in=\angle] (join) 
    to[out=\s*90, in=-\s*90] (exit);
}


\newcommandx{\strJoin}[7][1=,2=,4=0.5,5=0.5,7=,usedefault]{
    \drawFork[#1][#2]{#3}[-#4][-#5][#7]
    \coordinate (#6) at (exit);
}

\newcommandx{\strSplit}[8][1=,2=,4=0.5,5=0.5,7=1,8=]{
    \getNodes{#6}{\splitNodes}
    \tikzmath{
        \s=#4+#5;
    }
    \splitTargets{#3}{\splitNodes}{#7}{\s}
    \drawFork[#1][#2]{#6}[#5][#4][#8]
}

\newcommandx{\strMod}[8][1=,2=,3=,5=0.5,7=0.5,usedefault]{
    \coordinate[shift={(0,-#5)}] (joint) at (#4);

    \listLengthX{#1,#2}{\lflen}
    \listLengthX{#1,#3}{\rtlen}

    \tikzmath{
        \TCWidth=10+symWidth(0,\lflen,\rtlen);    
    }
    \draw (joint) node[mod={\TCWidth}](joint){#6};
    
    \ifdim #5 pt > 0 pt
        \coordinate (entry) at (#4);
        \xdef\modPathL{
            (entry)--(entry|-joint.north)-|(joint.south west)
        }
        \xdef\modPathR{
            (entry)--(entry|-joint.north)-|(joint.south east)
        }
    \else
        \coordinate (entry) at (joint.north);
        \xdef\modPathL{
            (joint.north)-|(joint.south west)
        }
        \xdef\modPathR{
            (joint.north)-|(joint.south east)
        }
    \fi

    \ifdim #7 pt > 0 pt
        \coordinate[shift={(0,-#7)}] (exit) at (joint);
        \coordinate (#8) at (exit);
        \xdef\modPathL{\modPathL-|(exit)}
        \xdef\modPathR{\modPathR-|(exit)}
    \else
        \coordinate (exit) at (joint.south);
        \xdef\modPathL{\modPathL-|(exit)}
        \xdef\modPathR{\modPathR-|(exit)}
    \fi

    \highlightSide{#1}{#2}{
        \modPathL
    }{
        --++(0,-3)
        -|($(joint.west)+(-3,0)$)
        |-($(entry)+(0,3)$)
        --(entry)
    }
    \draw[NTDash, rounded corners=0.5,line width=\lineWidth] \modPathL;

    \reverseList{#3}{\rNTCol}
    \highlightSide{#1}{\rNTCol}{
        \modPathR
    }{
        --++(0,-3)
        -|($(joint.east)+(3,0)$)
        |-($(entry)+(0,3)$)
        --(entry)
    }
    \draw[NTDash, rounded corners=0.5, line width=\lineWidth] \modPathR;
}

\newcommandx{\strTwoCell}[8][1=,3=0.5,5=0,6=0.5,8=,usedefault]{

    \readlist*\lst{#2}
    \readlist*\outlst{#7}
    \getNodes{#2}{\nodes}
    \joinTarget{\nodes}{-#3}{joint}[\nodesWidth]

    \listLengthX{\lst[1,2],\lst[1,3]}{\lflen}
    \listLengthX{\lst[-1,2],\lst[-1,4]}{\rtlen}
    \listLengthX{\outlst[1,2],\lst[1,3]}{\lflenII}
    \listLengthX{\outlst[-1,2],\lst[-1,4]}{\rtlenII}

    \tikzmath{
        \lshft=TCLShft(\lflen);
        \rshft=-TCLShft(\rtlen);
        \TCWidth=10+max(symWidth(\nodesWidth,\lflen,\rtlen),symWidth(((#5)*28.45276),\lflenII, \rtlenII));
    }
    \draw (joint) node[twocellX={\TCWidth}](joint){#4};


    \foreach \i in {1,...,\lstlen}{
        \ifnum \i=1 then
            \coordinate[xshift=\lshft] (hlcursor) at (\lst[1,1]);
            \clipS{hlcursor}{joint.west}
            \highlightSide{#1}{}{
                (hlcursor)
                --(hlcursor|-joint.north)
                -|(joint.west)
            }{\leftClip}
        \fi

        \ifnum \i=\lstlen then
            \coordinate[xshift=\rshft] (hlcursor) at (\lst[-1,1]);
            \clipS{hlcursor}{joint.east}
            \highlightSide{#1}{}{
                (hlcursor)
                --(hlcursor|-joint.north)
                -|(joint.east)
            }{\rightClip}

            \edef\fCol{\lst[-1,2]}
            \edef\lntCol{\lst[-1,3]}
            \edef\rntCol{\lst[-1,4]}

            \strIdTo{\lst[-1,1]}{joint}[\fCol][\lntCol][\rntCol]
        \else
            \listLengthX{\lst[\i,2],\lst[\i,4]}{\rtlen}
            \listLengthX{\lst[\i+1,2],\lst[\i+1,3]}{\lflen}

            \tikzmath{
                \rshft=-TCLShft(\rtlen);
                \lshft=TCLShft(\lflen);
            }

            \coordinate[xshift=\rshft] (hlcursor) at (\lst[\i,1]);
            \coordinate[xshift=\lshft] (hlcursor2) at (\lst[\i+1,1]);

            \highlightSide{#1}{}{
                (hlcursor)
                --(hlcursor|-joint.north)
                -|(hlcursor2)
            }{--++(0,3)
            -| (hlcursor)}

            \edef\fCol{\lst[\i,2]}
            \edef\lntCol{\lst[\i,3]}
            \edef\rntCol{\lst[\i,4]}

            \strIdTo{\lst[\i,1]}{joint}[\fCol][\lntCol][\rntCol]
        \fi
    }    

    \getNodes{#7}{\outNodes}
    \splitTargets{joint}{\outNodes}{#5}{#6}

    \foreach \i in {1,...,\outlstlen}{
        \ifnum \i=1 then
            \listLengthX{\outlst[1,2],\outlst[1,3]}{\lflen}

            \tikzmath{
                \lshft=TCLShft(\lflen);
            }
            \coordinate[xshift=\lshft] (hlcursor) at (\outlst[1,1]);
            \clipS{hlcursor}{joint.west}
            \highlightSide{#1}{}{
                (hlcursor)
                --(hlcursor|-joint.south)
                -|(joint.west)
            }{\leftClip}
        \fi

        \ifnum \i=\outlstlen then
            \listLengthX{\outlst[-1,2],\outlst[-1,4]}{\rtlen}

            \tikzmath{
                \rshft=-TCLShft(\rtlen);
            }
            \coordinate[xshift=\rshft] (hlcursor) at (\outlst[-1,1]);
            \clipS{hlcursor}{joint.east}
            \highlightSide{#1}{}{
                (hlcursor)
                --(hlcursor|-joint.south)
                -|(joint.east)
            }{\rightClip}

            \edef\fCol{\outlst[-1,2]}
            \edef\lntCol{\outlst[-1,3]}
            \edef\rntCol{\outlst[-1,4]}

            \drawS{joint-|\outlst[\i,1]}{\outlst[\i,1]}[\fCol][\lntCol][\rntCol]
        \else
            \listLengthX{\outlst[\i,2],\outlst[\i,4]}{\rtlen}
            \listLengthX{\outlst[\i+1,2],\outlst[\i+1,3]}{\lflen}

            \tikzmath{
                \rshft=-TCLShft(\rtlen);
                \lshft=TCLShft(\lflen);
            }

            \coordinate[xshift=\rshft] (hlcursor) at (\outlst[\i,1]);
            \coordinate[xshift=\lshft] (hlcursor2) at (\outlst[\i+1,1]);

            \highlightSide{#1}{}{
                (hlcursor)
                --(hlcursor|-joint.south)
                -|(hlcursor2)
            }{--++(0,-3)
                -| (hlcursor)
            }

            \edef\fCol{\outlst[\i,2]}
            \edef\lntCol{\outlst[\i,3]}
            \edef\rntCol{\outlst[\i,4]}

            \drawS{joint-|\outlst[\i,1]}{\outlst[\i,1]}[\fCol][\lntCol][\rntCol]
        \fi
    }
    \draw (joint) node[twocellX={\TCWidth}](joint){#4};
}

\newcommandx{\idCup}[2]{
    \xdef\colours{#2}        
    \listLength{\colours}{\colourslen}
    \foreach \c [count=\k] in \colours{
        \tikzmath{
            real \rad;
            \rad=idRad(\colourslen-\k+1);
        }
        \coordinate[xshift=-\rad pt
        ] (temp) at (#1);
        \draw[
            line width=\hlWidth pt,
            color=\c
        ]
        (temp) arc(180:360:\rad pt);
    }
}

\newcommandx{\idCap}[2]{
    \xdef\colours{#2}        
    \listLength{\colours}{\colourslen}
    \foreach \c [count=\k] in \colours{
        \tikzmath{
            real \rad;
            \rad=idRad(\colourslen-\k+1);
        }
        \coordinate[xshift=\rad pt
        ] (temp) at (#1);
        \draw[
            line width=\hlWidth pt,
            color=\c
        ]
        (temp) arc(0:180:\rad pt);
    }
}

\newcommandx{\strKey}[1]{
    \readlist*\keyIn{#1}
    \coordinate (currentNode) at (current bounding box.north);
    \begin{scope}[local bounding box=outer box]
        \foreach \i in {\keyInlen,...,1}{
            \edef\nodeName{\keyIn[\i,1]}
            \edef\nodeColour{\keyIn[\i,2]}
        
            \coordinate (temp) at (currentNode);
            \coordinate[shift={(0,0.5)}] (currentNode) at (temp);

            \draw (currentNode) node[label, anchor=east](temp){\nodeName};
            \draw[color=\nodeColour, line width=\hlWidth] (currentNode) --++(0.3,0);
        }   
    \end{scope}
    \coordinate[shift={(0.1,0)}] (topRight) at (outer box.north east);
    \draw[black] (outer box.south west) rectangle (topRight);
}

\newcommandx{\strKeyX}[1]{
    \readlist*\keyIn{#1}
    \tikzset{
        key/.pic={    
            \coordinate (currentNode) at (0,0);
            \begin{scope}[local bounding box=outer box]
                \foreach \i in {\keyInlen,...,1}{
                    \edef\nodeName{\keyIn[\i,1]}
                    \edef\nodeColour{\keyIn[\i,2]}
        
                    \coordinate (temp) at (currentNode);
                    \coordinate[shift={(0,0.5)}] (currentNode) at (temp);

                    \draw (currentNode) node[label, anchor=east](temp){\nodeName};
                    \draw[color=\nodeColour, line width=\hlWidth] (currentNode) --++(0.3,0);
                }  
            \end{scope}
            \coordinate[shift={(0.1cm,0)}] (topRight) at (outer box.north east);
            \draw[black] (outer box.south west) rectangle (topRight);
        }
    }
    \draw (current bounding box.north) pic{key};
}

\newcommandx{\strKeyXX}[1]{
    \readlist*\keyIn{#1}
    \draw (current bounding box.north) node[label, anchor=south]{
            \begin{tikzpicture}
                \coordinate (currentNode) at (0,0);
                \begin{scope}[local bounding box=outer box]
                    \foreach \i in {\keyInlen,...,1}{
                        \edef\nodeName{\keyIn[\i,1]}
                        \edef\nodeColour{\keyIn[\i,2]}
            
                        \coordinate (temp) at (currentNode);
                        \coordinate[shift={(0,0.5)}] (currentNode) at (temp);
    
                        \draw (currentNode) node[label, anchor=east](temp){\nodeName};
                        \draw[color=\nodeColour, line width=\hlWidth] (currentNode) --++(0.3,0);
                    }  
                \end{scope}
                \coordinate[shift={(0.1cm,0)}] (topRight) at (outer box.north east);
                \draw[black] (outer box.south west) rectangle (topRight);
            \end{tikzpicture}
    };
}

\newcommandx{\strLabel}[6][3=,4=,5=,6=1]{
    \tikzmath{
        \height=0.5*#6;
    }
    \coordinate[shift={(0,-\height)}] (labelTemp) at (#1);
    \strId{#1}[#3][#4][#5][#6]
    \draw (labelTemp) node[label]{#2};    
}



==> stringmacros.tex <==
\newcommandx{\stringTwoTone}[6][6=]{
    \ifthenelse{\equal{#6}{}}{
        \tikzset{
            optionZero/.style={
                line width=2pt, color=white
            },
            optionOne/.style={
                line width=2pt, color=#2
            },
            optionTwo/.style={
                line width=2pt, color=#3
            }
        }
    }
    {
        \tikzset{
            optionZero/.style={
                very thick, draw=white, double=white, double distance=2pt
            },
            optionOne/.style={
                very thick, draw=white, double=#2, double distance=2pt
            },
            optionTwo/.style={
                very thick, draw=white, double=#3, double distance=2pt
            }
        }
    }
    \begin{scope}
        \draw[optionZero] #1;
    \end{scope}
    \begin{scope}[overlay]
        \clip #1 #4;
        \draw[optionOne] #1;
    \end{scope}
    \begin{scope}[overlay]
        \clip #1 #5;
        \draw[optionTwo] #1;
    \end{scope}
    \begin{scope}[]
        \draw[thin, white] #1;
    \end{scope}
}
\newcommandx{\stringLeftBraid}[5][5=1]{
\setsepchar{,}
\readlist*\inputSLB{#1}
\readlist*\output{#2}
\readlist*\colours{#3}

\gettikzxy{(\inputSLB[1])}{\ax}{\ay}
\gettikzxy{(\inputSLB[2])}{\bx}{\by}
  
\pgfmathsetmacro\xCoord{(\ax+\bx)/2}
\pgfmathsetmacro\yCoord{min(\ay,\by)}

\coordinate (temp1) at ($(\xCoord pt,\yCoord pt)-(0,0.5*#5)$);

\pgfmathsetmacro\xCoord{min(\ax,\bx)}

\coordinate (temp2) at ($(\xCoord pt,\yCoord pt)-(0,#5)$);

\pgfmathsetmacro\xCoord{max(\ax,\bx)}

\coordinate (temp3) at ($(\xCoord pt,\yCoord pt)-(0,#5)$);

\draw[thick,color=#4] (\inputSLB[2]) to[only out=-90] (temp1);

\draw[thick,color=#3] (temp1) to[only in=90] (temp2);

\stringTwoTone{(\inputSLB[1]) to [out=-90,in=90] (temp3)} {#4}{#3}{
    --++(0,-2)
    --++(2,0)
    --($(\inputSLB[2])+(2,2)$)
    --($(\inputSLB[1])+(0,2)$)
    --++(0,-2)
}{
    --++(0,-2)
    --($(temp2)+(-2,-2)$)
    --($(\inputSLB[1])+(-2,2)$)
    --++(2,0)
    --++(0,-2)
}[
    braid
]
\coordinate (\output[1]) at (temp2);
\coordinate (\output[2]) at (temp3);
}
\newcommandx{\stringRightBraid}[5][5=1]{
    \setsepchar{,}
    \readlist*\inputSRB{#1}
    \readlist*\output{#2}
    \readlist*\colours{#3}
    
    \gettikzxy{(\inputSRB[1])}{\ax}{\ay}
    \gettikzxy{(\inputSRB[2])}{\bx}{\by}
      
    \pgfmathsetmacro\xCoord{(\ax+\bx)/2}
    \pgfmathsetmacro\yCoord{min(\ay,\by)}
    
    \coordinate (temp1) at ($(\xCoord pt,\yCoord pt)-(0,0.5*#5)$);

    \pgfmathsetmacro\xCoord{min(\ax,\bx)}

    \coordinate (temp2) at ($(\xCoord pt,\yCoord pt)-(0,#5)$);

    \pgfmathsetmacro\xCoord{max(\ax,\bx)}

    \coordinate (temp3) at ($(\xCoord pt,\yCoord pt)-(0,#5)$);
    
    \draw[thick,color=#3] (\inputSRB[1]) to[only out=-90] (temp1);
    
    \draw[thick,color=#4] (temp1) to[only in=90] (temp3);
    
    \stringTwoTone{
        (\inputSRB[2]) to[out=-90, in=90] (temp2)
        }{#4}{#3}{
        --++(0,-2)
        --($(temp3)+(2,-2)$)
        --($(\inputSRB[2])+(2,2)$)
        --++(-2,0)
        --++(0,-2)
    }{
        --++(0,-2)
        --++(-2,0)
        --($(\inputSRB[1])+(-2,2)$)
        --($(\inputSRB[2])+(0,2)$)
        --++(0,-2)
    }[
        braid
    ]
    \coordinate (\output[1]) at (temp2);
    \coordinate (\output[2]) at (temp3);
}

\newcommandx{\stringCapCC}[6][]{
    \readlist*\outputnodes{#2}
    \coordinate (temp1) at ($(#1)+(-0.5*#3,-#4)$);
    \coordinate (temp2) at ($(#1)+(0.5*#3,-#4)$);
    \stringTwoTone{
        (temp1) to[out=90, in=180] (#1)
        to [out=0, in=90] (temp2)
    }{#5}{#6}
    {
        --++(0,-1)
        --++(4,0)
        --++(0,#4)
        --++(0,3)
        --++(-#3,0)
        --++(-8,0)
        --++(0,-3)
        --++(0,-#4)
        --++(4,0)
        --++(0,1)
    }
    {
        --++(0,-1)
        --++(#3,0)
        --++(0,1)
    }
    \coordinate (\outputnodes[1]) at (temp1);
    \coordinate (\outputnodes[2]) at (temp2);
}
\newcommandx{\stringCapC}[5]{
    \readlist*\outputnodes{#2}
    \coordinate (temp1) at ($(#1)+(-0.5*#3,-#4)$);
    \coordinate (temp2) at ($(#1)+(0.5*#3,-#4)$);
    \draw[thick,#5] (temp1) to[out=90, in=180] (#1)
        to [out=0, in=90] (temp2);
    \coordinate (\outputnodes[1]) at (temp1);
    \coordinate (\outputnodes[2]) at (temp2);
}

\newcommandx{\stringCap}[5][3=1,4=0.5,5=black,usedefault]{
    \setsepchar{,}
    \readlist*\colours{#5}
    \ifthenelse{\colourslen>1}{
        \xdef\colourOne{\colours[1]}
        \xdef\colourTwo{\colours[2]}
        \stringCapCC{#1}{#2}{#3}{#4}{\colourOne}{\colourTwo}
    }{
        \xdef\colourOne{\colours[1]}
        \stringCapC{#1}{#2}{#3}{#4}{\colourOne}
    }
}
\newcommandx{\stringCup}[3][2=0.5,3=black,usedefault]{
    \readlist*\inputStringCup{#1}
    \coordinate (temp1) at (\inputStringCup[1]);
    \coordinate (temp3) at (\inputStringCup[2]);

    \gettikzxy{(\inputStringCup[1])}{\ax}{\ay}
    \gettikzxy{(\inputStringCup[2])}{\bx}{\by}
      
    \pgfmathsetmacro\xCoord{(\ax+\bx)/2}
    \pgfmathsetmacro\yCoord{min(\ay,\by)}

    \coordinate (temp2) at ($(\xCoord pt,\yCoord pt)+(0,-#2)$);

    \readlist*\colours{#3}
    \ifthenelse{\colourslen>1}{
        \xdef\colourOne{\colours[1]}
        \xdef\colourTwo{\colours[2]}
    \stringTwoTone{
        (temp1) to[out=-90, in=180] (temp2)
        to[out=0, in=-90] (temp3)
    }{\colourOne}{\colourTwo}
    {
        --++(0,2)
        --++(2,0)
        --($(temp2)+(\xCoord pt,-2)+(2,0)$)
        --($(temp2)+(-\xCoord pt,-2)-(2,0)$)
        --($(temp1)+(-2,2)$)
        --++(2,0)
        --++(0,-2)
    }
    {
        --++(0,2)
        --($(temp1)+(0,2)$)
        --++(0,-2)
    }
    }{
        \xdef\colourOne{\colours[1]}
        \draw[thick, \colourOne] (temp1) to[out=-90, in=180] (temp2) to[out=0, in=-90] (temp3);
    }
}

\newcommandx{\stringIdCC}[4][4=1]{
    \coordinate (temp1) at ($(#1)+(0,-#4)$);
    \stringTwoTone{
        (#1)to[out=-90,in=90](temp1)
        }{#2}{#3}{
        --++(0,-1)
        --++(-10,0)
        --++(0,2)
        --++(0,#4)
        --++(10,0)
    }
    {
        --++(0,-1)
        --++(10,0)
        --++(0,2)
        --++(0,#4)
        --++(-10,0)
    }[]
    \coordinate(#1) at (temp1);
}
\newcommandx{\stringIdC}[3][3=1]{
    \coordinate (temp1) at ($(#1)+(0,-#3)$);
    \draw [color=#2, thick] (#1) to (temp1);
    \coordinate (#1) at (temp1);
}

\newcommandx{\stringId}[3][2=1,3=black,usedefault]{
    \setsepchar{,}
    \readlist*\colours{#3}
    \ifthenelse{
        \colourslen>1
    }{
        \xdef\colourOne{\colours[1]}
        \xdef\colourTwo{\colours[2]}
        \stringIdCC{#1}{\colourOne}{\colourTwo}[#2]
    }{
        \xdef\colourOne{\colours[1]}
        \stringIdC{#1}{\colourOne}[#2]
    }
}

\newcommandx{\colourChange}[5][4=0.5,5=0.5]{
    \stringId{#1}[#4][#2]
    \coordinate (temp11) at (#1);
    \stringId{#1}[#5][#3]
    \draw (temp11) node[bullet]{};
}
\newcommandx{\stringLabel}[5][4=0.5,5=0.5]{
    \stringId{#1}[#4][#2]
    \coordinate (temp11) at (#1);
    \stringId{#1}[#5][#2]
    \draw (temp11) node[label]{#3};
}

\newcommandx{\clipPathS}[2]{
    \gettikzxy{(#1)}{\xTop}{\yTop}
    \gettikzxy{(#2)}{\xBottom}{\yBottom}

    \newdimen \xTopDim
    \xTopDim = \xTop pt
    \newdimen \xBottomDim
    \xBottomDim =\xBottom pt

    \ifthenelse{
        \lengthtest{\xTopDim <\xBottomDim}
    }{
        \xdef\leftClipPath{
            --++(0,-2)
            --($(\xTop,\yBottom)+(-2,-2)$)
            --($(#1)+(-2,2)$)
            --++(2,0)
            --++(0,-2)
        }
        \xdef\rightClipPath{
            --++(0,-2)
            --++(2,0)
            --($(\xBottom, \yTop)+(2,2)$)
            --($(#1)+(0,2)$)
            --++(0,-2)
        }
    }{
        \xdef\leftClipPath{
            --++(0,-2)
            --++(-2,0)
            --($(\xBottom, \yTop)+(-2,2)$)
            --($(#1)+(0,2)$)
            --++(0,-2)
        }  
        \xdef\rightClipPath{
            --++(0,-2)
            --($(\xTop,\yBottom)+(2,-2)$)
            --($(#1)+(2,2)$)
            --++(-2,0)
            --++(0,-2)
        }
    }
}
\newcommandx{\stringTwoCell}[7][1=0.5,5=0,6=0.5,7=twocell,usedefault]{
    \setsepchar[.]{,./}
    \readlist*\inputs{#2}
    \xdef\xCoordinateList{}
    \xdef\yCoordinateList{}
    \foreach \index in {1,...,\inputslen}{
        \gettikzxy{(\inputs[\index,1])}{\ax}{\ay}
        \xdef\xCoordinateList{\ax,\xCoordinateList}
        \xdef\yCoordinateList{\ay,\yCoordinateList}
    }
    \pgfmathsetmacro\minX{min(\xCoordinateList)}
    \pgfmathsetmacro\maxX{max(\xCoordinateList)}
    \pgfmathsetmacro\xCoordinate{(\maxX+\minX)/2}
    \pgfmathsetmacro\yCoordinate{min(\yCoordinateList)}
    
    \coordinate (temp1) at (\xCoordinate pt, \yCoordinate pt);
    \coordinate (temp1) at ($(temp1)+(0,-#1)$);
    
    \pgfmathsetmacro\startAngle{180*(1-(1/(2*\inputslen)))}
    \pgfmathsetmacro\increaseAngle{180/(\inputslen)}
    \foreach \index in {1,...,\inputslen}{
        \xdef\currentPath{
            (\inputs[\index,1]) to[out=-90, in=\angle] (temp1)
        }
        \pgfmathsetmacro\angle{\startAngle+((1-\index)*\increaseAngle)}
        \ifthenelse{\listlen\inputs[\index]=1}{
            \draw[thick,black] \currentPath;
        }{}
        \ifthenelse{\listlen\inputs[\index]=2}{
            \xdef\currentColour{\inputs[\index,2]}
            \tikzset{
                workAround/.style={
                    thick,
                    color=\currentColour
                }
            }
            \draw[workAround] \currentPath;
        }{}
        \ifthenelse{\listlen\inputs[\index]>2}{
            \xdef\colourOne{\inputs[\index,2]}
            \xdef\colourTwo{\inputs[\index,3]}
            
            \clipPathS{\inputs[\index,1]}{temp1}

            \stringTwoTone{\currentPath}{\colourOne}{\colourTwo}{
                \leftClipPath;
            }
            {
                \rightClipPath;
            }
        }{}
    }
    \ifthenelse{\equal{#4}{}}{
    }
    {
    \readlist*\outputs{#4}
    \draw (temp1)++(-0.5*#5,-#6) node [blank] (temp2){};
    
    \pgfmathsetmacro\startAngle{180*((1/(2*\outputslen))-1)}
    \pgfmathsetmacro\increaseAngle{180/(\outputslen)}

    \ifthenelse{\outputslen>1}{
    \def\outputspace{
        {#5/(\outputslen-1)}}
    }{
        \def\outputspace{0}
    }

    \foreach \index in {1,...,\outputslen}{
        \pgfmathsetmacro\angle{\startAngle+((\index-1)*\increaseAngle)}

        \draw (temp2) node[blank] (\outputs[\index,1]){};
        \xdef\currentPath{
            (temp1) to[out=\angle, in=90] (\outputs[\index,1])
        }
        \ifthenelse{\listlen\outputs[\index]=1}
        {
            \draw[thick,black] \currentPath;
        }{}
        \ifthenelse{\listlen\outputs[\index]=2}{
            \xdef\currentColour{\outputs[\index,2]}
            \tikzset{
                workAround/.style={
                    thick,
                    color=\currentColour
                }
            }
            \draw[workAround] \currentPath;
        }{}
        \ifthenelse{\listlen\outputs[\index]>2}{
            \xdef\colourOne{\outputs[\index,2]}
            \xdef\colourTwo{\outputs[\index,3]}
            
            \clipPathS{temp1}{\outputs[\index,1]}

            \stringTwoTone{\currentPath}{\colourOne}{\colourTwo}{
                \leftClipPath;
            }
            {
                \rightClipPath;
            }
        }{}
        \draw (temp2)++({\outputspace},0) node[blank] (temp2){};
    }
    }
    \draw (temp1) node[#7](temp1){#3};
    \setsepchar[.]{,./}
}



==> tikzmacros.tex <==
\definecolor{cb-orange}{cmyk}{0,0.5,1,0}
\definecolor{cb-light-blue}{cmyk}{0.8,0,0,0}
\definecolor{cb-green}{cmyk}{0.97,0,0.75,0}
\definecolor{cb-yellow}{cmyk}{0.1,0.05,0.9,0}
\definecolor{cb-blue}{cmyk}{1,0.5,0,0}
\definecolor{cb-red}{cmyk}{0,0.8,1,0}
\definecolor{cb-pink}{cmyk}{0.1,0.7,0,0}

\definecolor{cb-purple}{RGB}{62,35,115}

\definecolor{alt-plum}{RGB}{51,34,136}
\definecolor{alt-green}{RGB}{17,119,51}
\definecolor{alt-turq}{RGB}{68,170,153}
\definecolor{alt-blue}{RGB}{136,204,238}
\definecolor{alt-yellow}{RGB}{221,204,119}
\definecolor{alt-pink}{RGB}{204,102,119}
\definecolor{alt-purple}{RGB}{170,68,153}
\definecolor{alt-red}{RGB}{136,34,85}

\colorlet{c1}{cb-orange}
\colorlet{c2}{cb-light-blue}
\colorlet{c3}{cb-green}
\colorlet{c4}{cb-pink}
\colorlet{c5}{cb-blue}
\colorlet{c6}{cb-red}
\colorlet{c7}{cb-yellow}
\colorlet{c8}{alt-red}

\tikzset{
  blank/.style={
    inner sep = 0cm, 
    outer sep = 0cm, 
    align=center, 
    minimum size=0pt
  },
  label/.style={
    minimum size=5mm, 
    inner sep=0.1cm,
    fill=white
  },
  midarrow/.style={
    currarrow,
    sloped,
    scale=0.5,
    allow upside down
  },
  shorten <>/.style={
    shorten >=#1,
    shorten <=#1
  },
  bullet/.style={
    rectangle,
    draw,
    fill=black,
    minimum size=3pt,
    inner sep=0pt,
  },
  colourBullet/.style={
    circle,
    draw=#1,
    fill=#1,
    minimum size=3pt,
    inner sep=0pt,
  },
  double colour/.style 2 args={fill=#1, 
  path picture={
    \fill[#2, sharp corners] 
    (path picture bounding box.south) -|
    (path picture bounding box.north east) --
    (path picture bounding box.north) --
    cycle;
    }
  },
  modification/.style 2 args={
    rounded corners=2,
    double colour={#1}{#2},
    minimum size=5mm,
    inner sep = 0.1cm, 
    outer sep = 0cm, 
    align=center,
    text=white
  },
  functorNode/.style={
    modification={#1}{#1}
  },
  twocellarr/.style={
    shorten <= 10pt, 
    shorten >= 10pt
  },
  twocell/.style={
    functorNode={black}
  },
  twocellX/.style ={
    rectangle,
    thick,
    fill=white,
    rounded corners=0.5,
    inner sep = 0.1cm, 
    outer sep = 0cm, 
    align=center,
    minimum width={#1 pt},
    draw=black,
    line width=\lineWidth
    },
  mod/.style ={
    rectangle,
    thick,
    fill=white,
    rounded corners=0.5,
    inner sep = 0.1cm, 
    outer sep = 0cm, 
    align=center,
    minimum width={#1 pt},
  },
  mod2/.style ={
    rectangle,
    dashed,
    thick,
    fill=white,
    rounded corners=0.5,
    inner sep = 0.1cm, 
    outer sep = 0cm, 
    align=center,
    minimum width={#1 pt},
  },
  colChange/.style ={
    rectangle,
    thick,
    fill=black,
    rounded corners=0.5,
    inner sep = 0.1cm, 
    outer sep = 0cm, 
    align=center,
    minimum width={#1 pt},
  },
  only in/.style={
    to path={
      let
      \p1 = ($ (\tikztotarget) - (\tikztostart) $)
      in
      .. controls 
      ($(\tikztostart)!{veclen(\x1,\y1)/3}!($(\tikztotarget)+(#1:{veclen(\x1,\y1)/3})$)$)
      and
      ($(\tikztotarget)+(#1:{veclen(\x1,\y1)/3})$)
      .. (\tikztotarget)
    }
  },
  only out/.style={
    \path draw (\tikztostart) --node[](temp1){} (\tikztotarget-|)
    to path={
      let
      \p1 = ($ (\tikztotarget) - (\tikztostart) $)
      in
      .. controls 
      ($(\tikztostart)+(#1:{veclen(\x1,\y1)/3})$)
      and
      ($(\tikztotarget)!{veclen(\x1,\y1)/3}!($(\tikztostart)+(#1:{veclen(\x1,\y1)/3})$)$)
      .. (\tikztotarget)
    }
  },
  braidTop/.style={
    to path={
      let
      \p1=($(\tikztotarget)-(\tikztostart)$)
      in
      ..controls +(0,\y1/2).. (\tikztotarget)
    }
  },
  braidBottom/.style={
    to path={
      let
      \p1=($(\tikztotarget)-(\tikztostart)$)
      in
      ..controls +(\x1/2,0).. (\tikztotarget)
    }
  },
  NTDash/.style={
    dash pattern= on 0.20cm off 0.05cm,
  },
}
\makeatletter
\newcommand{\gettikzxy}[3]{%
    \tikz@scan@one@point\pgfutil@firstofone#1\relax
    \edef#2{\the\pgf@x}%
    \edef#3{\the\pgf@y}%
}
\makeatother
\newcommand{\drawCrossing}[2]{
    \draw (#1)++(0,-1) node[blank] (temp1){};
    \draw (#2)++(0,-1) node[blank] (temp2){};

    \draw[thick,black] (#1) to[out=-90, in=90] (temp2) node [blank] (#1){};
    \draw[thick,black] (#2) to[out=-90, in=90] (temp1) node [blank] (#2){};
}

\newcommand{\drawBraid}[2]{
    \draw (#1)++(0,-1) node[blank] (temp1){};
    \draw (#2)++(0,-1) node[blank] (temp2){};
  
    \strand[thick,black] (#1) to[out=-90, in=90] (temp2) node [blank] (#1){};
    \strand[thick,black] (#2) to[out=-90, in=90] (temp1) node [blank] (#2){};
}

\newcommand{\drawStraightDown}[2][1]{
  \strand[thick,black] (#2) to[out=-90, in=90] ++(0,-#1) node[blank] (#2){};
}

\newcommandx{\drawStraightDownX}[2][1=1]{
  \foreach \i in {#2}{
    \draw[thick,black] (\i) to[out=-90, in=90] ++(0,-#1) node[blank] (\i){};
    }
}

\newcommandx{\drawId}[2][1=1]{
  \drawStraightDownX[#1]{#2}
}

\newcommandx{\drawBead}[5][1=0.5,4=0.5]{
    \draw[thick, black] (#2) to[out=-90, in=90] ++(0,-#1) node [twocell] {#3} to[out=-90, in=90] ++(0,-#4) node [blank] (#5){};
}

\newcommandx{\drawBeadBottom}[4][1=0.5]{
    \draw[thick, black] (#2) to[out=-90, in=90] ++(0,-#1) node [twocell](#4) {#3};
}

\newcommandx{\drawBeadTop}[4][3=0.5]{
    \drawBead[0]{#1}{#2}[#3]{#4}
}

\newcommandx{\drawCap}[7][2=1,3=1,6=,7=]{
    \draw (#1)++(#2,0) node[blank] (#4){};
    \draw (#4)++(0.5*#3,0.5) node[blank] (capTop){};
    \draw (#4)++(#3,0) node[blank] (#5){};

    \draw[thick,black] (#4) to[out=90, in=180] node[label,pos=0.1, anchor=east] {#6} (capTop);

    \draw[thick,black] (capTop) to[out=0, in=90] node[label,pos=0.9, anchor=west] {#7} (#5);
}

\newcommandx{\drawCup}[5][3=0.5,4=,5=,usedefault]{
    \path (#1) to node[pos=0.5, blank] (temp1){} (#2);
    \draw (temp1)++(0,-#3) node[blank] (temp2){};

    \strand[thick,black] (#1) to[out=-90, in=180] 
    node[label,pos=0.1, anchor=east] {#4} (temp2);

    \strand[thick,black] (temp2) to[out=0, in=-90] node[label,pos=0.9, anchor=west] {#5} (#2);
}

\newcommand{\drawLabel}[2]{
    \draw (#1) node[label, below] {#2};
}

\newcommand{\drawLabelAbove}[2]{
    \draw (#1) node[label, above] {#2};
}

\newcommand{\drawShift}[2]{
    \draw (#1)++(#2,-1) node [blank] (temp1){};
    \draw[thick,black] (#1) to[out=-90, in=90] (temp1) node [blank](#1){};
}
    
\newcommandx{\drawTwoToOne}[6][1=0.5,5=0.5]{
    \path (#2) to node[blank, pos=0.5] (temp1){} (#3);
    \draw (temp1)++(0,-#1) node[twocell](temp2){#4};

    \draw[thick,black] (#2) to [out=-90, in=135] (temp2);

    \draw[thick,black] (#3) to [out=-90, in=45] (temp2);

    \draw[thick,black] (temp2) to [out=-90, in=90] ++(0,-#5) node[blank](#6){};
}
\newcommandx{\drawOneToTwo}[7][1=0.5,4=1,5=0.5,usedefault]{
    \draw (#2)++(0,-#1) node[twocell] (temp1){#3};

    \draw[thick,black] (#2) to [out=-90, in=90] (temp1);

    \draw (temp1)++(-0.5*#4,-#5) node [blank] (#6){};
    \draw (temp1)++(0.5*#4,-#5) node [blank] (#7){};

    \draw[thick, black] (temp1) to [out=-135, in=90] (#6);

    \draw[thick,black]
      (temp1) to [out=-45, in=90] (#7);
}
\newcommand{\drawCombine}[3]{
    \path (#1) to node[blank, pos=0.5](temp1){} (#2);
    \draw (temp1)++(0,-0.5) node[blank](temp2){};

    \draw[thick,black] (#1) to [out=-90, in=135] (temp2);

    \draw[thick,black] (#2) to [out=-90, in=45] (temp2);

    \draw[thick,black]
      (temp2) to [out=-90, in=90] ++(0,-0.5) node[blank](#3){};
}

\newcommand{\drawSplit}[3]{
    \draw[thick,black] (#1) to[out=-90, in=90] ++(0,-0.5) node[blank] (temp1){};

    \draw[thick,black] (temp1) to[out=-135, in=90] ++(-0.5,-0.5) node[blank](#2){};

    \draw[thick,black] (temp1) to[out=-45, in=90] ++(0.5,-0.5) node[blank](#3){};
    }

\newcommandx{\drawTwoToTwo}[8][1=0.5,5=1,6=0.5]{
    \path (#2) to node[blank, pos=0.5] (temp1){} (#3);
    \draw (temp1)++(0,-#1) node[twocell](temp2){#4};

    \draw[thick,black] (#2) to [out=-90, in=135] (temp2);

    \draw[thick,black] (#3) to [out=-90, in=45] (temp2);

    \draw (temp2)++(-0.5*#5,-#6) node [blank] (#7){};
    \draw (temp2)++(0.5*#5,-#6) node [blank] (#8){};

    \draw[thick,black] (temp2) to [out=-135, in=90] (#7); 

    \draw[thick,black] (temp2) to [out=-45, in=90] (#8); 
}

    \newcommandx{\drawThreeToTwo}[9][1=0.5,6=1,7=0.5]{
      \path (#2) to node[blank, pos=0.5] (temp1){} (#4);
      \draw (temp1)++(0,-#1) node[twocell](temp2){#5};

      \draw[thick,black]
      (#2) to [out=-90, in=135] (temp2);

      \draw[thick,black]
      (#3) to [out=-90, in=90] (temp2);
      
      \draw[thick,black]
      (#4) to [out=-90, in=45] (temp2);
      
      \draw (temp2)++(-0.5*#6,-#7) node [blank] (#8){};
      \draw (temp2)++(0.5*#6,-#7) node [blank] (#9){};

      \draw[thick,black]
      (temp2) to [out=-135, in=90] (#8); 

      \draw[thick,black]
      (temp2) to [out=-45, in=90] (#9); 
    }
\newcommandx{\drawTwoCell}[6][1=0.5,5=0,6=0.5,usedefault]{
    \readlist*\inputs{#2}
    \xdef\xCoordinateList{}
    \xdef\yCoordinateList{}
    \foreach \index in {1,...,\inputslen}{
        \gettikzxy{(\inputs[\index])}{\ax}{\ay}
        \xdef\xCoordinateList{\ax,\xCoordinateList}
        \xdef\yCoordinateList{\ay,\yCoordinateList}
    }
    \pgfmathsetmacro\minX{min(\xCoordinateList)}
    \pgfmathsetmacro\maxX{max(\xCoordinateList)}
    \pgfmathsetmacro\xCoordinate{(\maxX+\minX)/2}
    \pgfmathsetmacro\yCoordinate{min(\yCoordinateList)}
    
    \coordinate (temp1) at (\xCoordinate pt, \yCoordinate pt);
    \coordinate (temp1) at ($(temp1)+(0,-#1)$);
    \draw (temp1) node[twocell](temp1){#3};
    
    \pgfmathsetmacro\startAngle{180*(1-(1/(2*\inputslen)))}
    \pgfmathsetmacro\increaseAngle{180/(\inputslen)}
    
    \foreach \index in {1,...,\inputslen}{
        \pgfmathsetmacro\angle{\startAngle+((1-\index)*\increaseAngle)}
        \draw[thick,black] (\inputs[\index]) to[out=-90, in=\angle] (temp1);
    }
    \draw (temp1) node[twocell](temp1){#3};

    \ifthenelse{\equal{#4}{}}{
    }
    {
    \readlist*\outputs{#4}
    \draw (temp1)++(-0.5*#5,-#6) node [blank] (temp2){};
    
    \pgfmathsetmacro\startAngle{180*((1/(2*\outputslen))-1)}
    \pgfmathsetmacro\increaseAngle{180/(\outputslen)}

    \ifthenelse{\outputslen>1}{
    \def\outputspace{
        {#5/(\outputslen-1)}}
    }{
        \def\outputspace{0}
    }

    \foreach \index in {1,...,\outputslen}{
        \pgfmathsetmacro\angle{\startAngle+((\index-1)*\increaseAngle)}

        \draw (temp2) node[blank] (\outputs[\index]){};
        \draw[thick,black] (temp1) to[out=\angle, in=90] (\outputs[\index]);
        
        \draw (temp2)++({\outputspace},0) node[blank] (temp2){};
    }
    }
}
    \newcommandx{\drawThreeToNone}[5][1=0.5]{
      \path (#2) to node[blank, pos=0.5] (temp1){} (#4);
      \draw (temp1)++(0,-#1) node[twocell](temp2){#5};

      \draw[thick,black]
      (#2) to [out=-90, in=135] (temp2);

      \draw[thick,black]
      (#3) to [out=-90, in=90] (temp2);
      
      \draw[thick,black]
      (#4) to [out=-90, in=45] (temp2);
    }
    \newcommand{\drawGeneralisedBraid}[2]{
      \drawTwoToTwo{#1}{#2}{$\chi$}[1]{#2}{#1}
    }
    \newcommandx{\drawCapX}[9][2=1,3=0.5,4=1,5=0.5,8=,9=, usedefault]{
      \newdimen \y
      \y = #2 pt
      \ifthenelse{\lengthtest{\y > 0pt}}{
      \draw (#1)++(#2,{#3-#5}) node[blank] (#6){};
      \draw (#1)++({#2+(0.5*#4)},#3) node[blank] (temp1){};
      \draw (#1)++({#2+#4},{#3-#5}) node[blank] (#7){};
      }
      {
        \draw (#1)++(#2,{#3-#5}) node[blank] (#7){};
        \draw (#1)++({#2-(0.5*#4)},#3) node[blank] (temp1){};
        \draw (#1)++({#2-#4},{#3-#5}) node[blank] (#6){};
      }
      \strand[thick,black] 
      (#6) to[out=90, in=180] 
      node[label,pos=0.1, anchor=east] {#8} (temp1);

      \strand[thick,black]
      (temp1) to[out=0, in=90] node[label,pos=0.9, anchor=west] {#9} (#7);
    }
    \newcommandx{\drawPositiveBraid}[6][3=1,4=-1,5=temp1,6=temp1,usedefault]{
      \path (#1) to node [pos=0.5, blank](temp1){} (#2);

      \draw (temp1)++(-0.5*#4,-#3) node[blank](temp2){};
      \draw (temp1)++(0.5*#4,-#3) node[blank](temp3){};

      \strand [thick,black]
      (#1) to[out=-90, in=90] (temp3);
      \strand [thick,black]
      (#2) to[out=-90, in=90] (temp2);

      \ifthenelse{\equal{#5}{temp1}}{
      \draw (temp2) node[blank] (#2){};
      \draw (temp3) node[blank] (#1){};
      }
      {
      \draw (temp2) node[blank] (#5){};
      \draw (temp3) node[blank] (#6){};
      }
    }
    \newcommandx{\drawNegativeBraid}[6][3=1,4=-1,5=temp1,6=temp1,usedefault]{
      \draw (#1)++(0,-#3) node[blank](temp2){};
      \draw (#2)++(0,-#3) node[blank](temp3){};

      
      \strand [thick,black]
      (#1) to[out=-90, in=90] (temp3);
      \strand [thick,black]
      (#2) to[out=-90, in=90] (temp2);

      \ifthenelse{\equal{#5}{temp1}}{
      \draw (temp2) node[blank] (#2){};
      \draw (temp3) node[blank] (#1){};
      }
      {
      \draw (temp2) node[blank] (#5){};
      \draw (temp3) node[blank] (#6){};
      }
    }
    \newcommandx{\drawBraidX}[6][3=1,4=-1,5=temp1,6=temp1,usedefault]{
      \newdimen \y
      \y = #4 pt
      \ifthenelse{\lengthtest{\y < 0pt}}
      {
        \drawNegativeBraid{#1}{#2}[#3][#4][#5][#6]
      }
      {
        \drawPositiveBraid{#1}{#2}[#3][#4][#5][#6]
      }
    }
    \newcommandx{\drawAcrossBraid}[2]{
      \draw (#1)++(0.2,0) node[blank](temp1){};
      \draw (#2)++(-0.2,0) node[blank](temp2){};

      \draw[thick, black](temp1) to [out=180, in=0] (temp2);
    }
    \newcommand{\drawStartNodes}[1]{
      \xdef\xCoord{0}
      \foreach \i/\j/\k in {#1}
      {
        \coordinate (\i) at (\xCoord,0);
        \draw (\i) node[label,anchor=south] {\j};
        \xdef\xCoord{\xCoord+\k}
      }
    }
    \newcommand{\drawEndNodes}[1]{
      \foreach \i/\j in {#1}
      {
        \draw(\i) node[label,anchor=north]{\j};
      }
    }
\newcommandx{\drawCapXX}[5]{
  \readlist*\feet{#4}
  \readlist*\feetlabels{#5}
  \coordinate (\feet[1]) at ($(#1)+(-0.5*#2,-#3)$);
  \coordinate (\feet[2]) at ($(#1)+(0.5*#2,-#3)$);

  \strand[thick,black]
    (\feet[1]) to[out=90, in=180] 
    node[pos=0.1, label] {\feetlabels[1]} (#1) 
    to[out=0, in=90] 
    node[pos=0.9, label]{\feetlabels[2]} (\feet[2]);
}
\newcommandx{\drawBraidLeft}[4]{
  \readlist*\inputDBL{#1}
  \readlist*\colours{#2}
  \readlist*\output{#4}
  \gettikzxy{(\inputDBL[1])}{\ax}{\ay}
  \gettikzxy{(\inputDBL[2])}{\bx}{\by}
  
  \pgfmathsetmacro\xCoord{(\ax+\bx)/2}
  \pgfmathsetmacro\yCoord{min(\ay,\by)}

  \coordinate (temp1) at ($(\xCoord pt,\yCoord pt)-(0,0.5*#3)$);

  \draw[thick, natTrans={green}{blue}]
  (\inputDBL[1]) to[out=-90, in=90] ($(\bx,\yCoord)-(0,#3)$) coordinate (\output[2]);

  \draw [shorten >= 0.2*#3,thick] 
  (\inputDBL[2]) to[out=-90, in=45] (temp1);

  \draw [shorten <= 0.2*#3, thick] 
  (temp1) to[only in=90] ($(\ax,\yCoord)-(0,#3)$) coordinate (\output[1]);
}
\newcommandx{\TwoTone}[6]{
  \xdef\tempPath{
    (#1) to[out=#2, in=#3] (#4)
  }
  \draw[very thick, color=#5] \tempPath;
  \begin{scope}[overlay]
    \clip  \tempPath --(20,0)--cycle;
    \draw[color=#6,very thick] \tempPath;
  \end{scope}
}

